Optimal Thermal Management, Charging, and Eco-driving of Battery Electric Vehicles

This paper addresses optimal battery thermal management (BTM), charging, and eco-driving of a battery electric vehicle (BEV) with the goal of improving its grid-to-meter energy efficiency. Thus, an optimisation problem is formulated, aiming at finding the optimal trade-off between trip time and charging cost. The formulated problem is then transformed into a hybrid dynamical system, where the dynamics in driving and charging modes are modeled with different functions and with different state and control vectors. Moreover, to improve computational efficiency, we propose modelling the driving dynamics in a spatial domain, where decisions are made along the traveled distance. Charging dynamics are modeled in a temporal domain, where decisions are made along a normalized charging time. The actual charging time is modeled as a scalar variable that is optimized simultaneously with the optimal state and control trajectories, for both charging and driving modes. The performance of the proposed algorithm is assessed over a road with a hilly terrain, where two charging possibilities are considered along the driving route. According to the results, trip time including driving and charging times, is reduced by 44 %, compared to a case without battery active heating/cooling.

==> bibliography_ah.tex <==
% A ------------------------------------------------------------------------------------
@article{abdollahi16,
  title={Optimal battery charging, Part I: Minimizing time-to-charge, energy loss, and temperature rise for OCV-resistance battery model},
  author={Abdollahi, Ali and Han, Xiaohong and Avvari, GV and Raghunathan, N and Balasingam, B and Pattipati, Krishna R and Bar-Shalom, Yaakov},
  journal={Journal of Power Sources},
  volume={303},
  pages={388--398},
  year={2016},
  publisher={Elsevier}
}

@MISC{advisor03,
  author =       {{ADVISOR}},
  organization = {National Renewable Energy Laboratory},
  title =        {Advanced Vehicle Simulator},
  howpublished = {\url{http://bigladdersoftware.com/advisor}},
  year =         {2003},
}

@ARTICLE{ahman01,
  author =       {Max \r{A}hman},
  title =        {Primary energy efficiency of alternative powertrains in vehicles},
  journal =      {Energy},
  year =         {2001},
  volume =       {26},
  number =       {11},
  pages =        {973-989},
}

@PHDTHESIS{alam14,
  author =       {Assad Alam},
  title =        {Fuel-efficient heavy-duty vehicle platooning},
  school =       {KTH},
  year =         {2014},
  address =      {Stockholm, Sweden},
}

@ARTICLE{alam14a,
  author =       {Assad Alam and Ather Gattami and Karl H. Johansson and Claire J. Tomlin},
  title =        {Guaranteeing safety for heavy duty vehicle platooning: Safe set computations and experimental evaluations},
  journal =      {Control Engineering Practice},
  year =         {2014},
  volume =       {24},
  pages =        {33-41},
}

@ARTICLE{alam15,
  author =       {Assad Alam and Jonas M\r{a}rtensson and Karl H. Johansson},
  title =        {Experimental evaluation of decentralized cooperative cruise control for heavy-duty vehicle platooning},
  journal =      {Control Engineering Practice},
  year =         {2015},
  volume =       {38},
  pages =        {11-25},
}

@ARTICLE{alam15b,
  author =       {Assad Alam and Bart Besselink and Jonas M\r{a}rtensson and Karl H. Johansson},
  title =        {Heavy-Duty Vehicle Platooning for Sustainable Freight Transportation: A Cooperative Method to Enhance Safety and Efficiency},
  journal =      {IEEE Control Systems Magazine},
  year =         {2015},
  volume =       {35},
  number =       {6},
  pages =        {34-56},
}

@TECHREPORT{alberer09,
  author =       {D. Alberer and L. Re},
  title =        {Optimization of the transient {D}iesel engine operation},
  institution =  {SAE International},
  type =         {Technical Paper},
  year =         {2009},
  number =       {2009-24-0113},
}

@ARTICLE{alberer09b,
  AUTHOR =       {D. Alberer and L. Re},
  TITLE =        {Fast Oxygen Based Transient {D}iesel Engine Operation},
  JOURNAL =      {SAE Int. J. Engines},
  YEAR =         {2009},
  volume =       {2},
  number =       {1},
  pages =        {405-413},
}

@TECHREPORT{altenstrasser12,
  author =       {Harald Altenstrasser and Yoshihisa Kato and Nikolaus Keuth and Thomas Winsel},
  title =        {{MiL}-Based Calibration and Validation of {D}iesel-{ECU} Models Using Emission and Fuel Consumption Prediction during Dynamic Warm-Up Tests ({NEDC})},
  institution =  {SAE International},
  type =         {Technical Paper},
  year =         {2012},
  number =       {2012-01-0432},
}

@ARTICLE{ambul09,
  author =       {Daniel Amb\"uhl and Lino Guzzella},
  title =        {Predictive reference signal generator for hybrid electric vehicles},
  journal =      {IEEE Transactions on Vehicular Technology},
  year =         {2009},
  volume =       {58},
  number =       {9},
  pages =        {4730-4740},
}

@ARTICLE{ambuhl10,
  AUTHOR =       {Daniel Amb\"uhl and Olle Sundstr\"om and Antonio Sciarretta and Lino Guzzella},
  TITLE =        {Explicit optimal control policy and its practical application for hybrid electric powertrains},
  JOURNAL =      {Control Engineering Practice},
  YEAR =         {2010},
  volume =       {18},
  number =       {12},
  pages =        {1429-1439},
}

@MANUAL{amesim,
  TITLE =        {{AMESim}},
  year =         {2010},
  note =         {\url{http://www.amesim.com/}},
}

@article{amini19,
  title={Cabin and battery thermal management of connected and automated HEVs for improved energy efficiency using hierarchical model predictive control},
  author={Amini, Mohammad Reza and Wang, Hao and Gong, Xun and Liao-McPherson, Dominic and Kolmanovsky, Ilya and Sun, Jing},
  journal={IEEE Transactions on Control Systems Technology},
  volume={28},
  number={5},
  pages={1711--1726},
  year={2019},
  publisher={IEEE}
}

@BOOK{anderson10,
  AUTHOR =       {Curtis D. Anderson and Judy Anderson},
  TITLE =        {Electric and Hybrid Cars, a History},
  PUBLISHER =    {McFarland \& Company, Inc.},
  YEAR =         {2010},
  edition =      {2},
}

@BOOK{andreasson05,
  AUTHOR =       {Niclas Andr\'easson and Anton Evgrafov and Michael Patriksson},
  TITLE =        {An Introduction to Continous Optimization},
  PUBLISHER =    {Studentlitteratur, Lund},
  YEAR =         {2005},
}

@article{andersson19,
  title={CasADi: a software framework for nonlinear optimization and optimal control},
  author={Andersson, Joel AE and Gillis, Joris and Horn, Greg and Rawlings, James B and Diehl, Moritz},
  journal={Mathematical Programming Computation},
  volume={11},
  number={1},
  pages={1--36},
  year={2019},
  publisher={Springer}
}

@ARTICLE{asprion14,
  author =       {Jonas Asprion and Oscar Chinellato and Lino Guzzella},
  title =        {Optimal control of diesel engines: numerical methods, applications, and experimental validation},
  journal =      {Math Probl Eng},
  year =         {2014},
  volume =       {},
  number =       {},
  pages =        {1-21},
}

@ARTICLE{assanis99,
  AUTHOR =       {D.~Assanis and G.~Delagrammatikas and R.~Fellini and Z.~Filipi and J.~Liedtke and N.~Michelena and P.~Papalambros and D.~Reyes and D.~Rosenbaum and A.~Sales and M.~Sasena},
  TITLE =        {An optimization approach to hybrid electric propulsion system design},
  JOURNAL =      {Journal of Mechanics of Structures and Machines, Automotive Research Center Special Edition},
  YEAR =         {1999},
  volume =       {27},
  number =       {4},
  pages =        {393-421},
}

@BOOK{atkins06,
  AUTHOR =       {Peter Atkins and Julio de Paula},
  TITLE =        {Physical Chemistry},
  PUBLISHER =    {W. H. Freeman},
  YEAR =         {2006},
  edition =      {8},
}

@TECHREPORT{atkinson05,
  author =       {C. Atkinson and G. Mott},
  title =        {Dynamic Model-Based Calibration Optimization: An Introduction and Application to {D}iesel Engines},
  institution =  {SAE International},
  type =         {Technical Paper},
  year =         {2005},
  number =       {2005-01-0026},
}

@TECHREPORT{atkinson08,
  author =       {C. Atkinson and M. Allain and H. Zhang},
  title =        {Using Model-Based Rapid Transient Calibration to Reduce Fuel Consumption and Emissions in {D}iesel Engines},
  institution =  {SAE International},
  type =         {Technical Paper},
  year =         {2008},
  number =       {2008-01-1365},
}

@MISC{audi,
  author =       {{Audi AG}},
  title =        {{Audi A1 e-tron}},
  howpublished = {\url{http://www.audi.com}},
  note =         {Accessed March 2012},
}

@TECHREPORT{autotram10,
  TITLE =        {{AutoTram}: Transport system of the future},
  INSTITUTION =  {Fraunhofer Institute for Transportation and Infrastructure Systems IVI},
  YEAR =         {2010},
}

@BOOK{astrom96,
  AUTHOR =       {Karl Johan Astrom and Bjorn Wittenmark},
  TITLE =        {Computer-Controlled Systems: Theory and Design},
  PUBLISHER =    {Prentice Hall},
  YEAR =         {1996},
}

% B ------------------------------------------------------------------------------------

@inproceedings{back02,
  address =      {Barcelona, Spain},
  author =       {M.~Back and M.~Simons and F.~Kirschbaum and V.~Krebs},
  booktitle =    {Proc. IFAC World Congress},
  title =        {{Predictive control of drivetrains}},
  year =         {2002},
  pages =        {1506-1506},
}

@BOOK{banish09,
  author =       {Greg Banish},
  title =        {Designing and Tuning High-Performance Fuel Injection Systems},
  publisher =    {CarTech},
  year =         {2009},
}

@Article{barkenbus2010eco,
  title={Eco-driving: An overlooked climate change initiative},
  author={Barkenbus, Jack N},
  journal={Energy Policy},
  volume={38},
  number={2},
  pages={762--769},
  year={2010},
  publisher={Elsevier}
}

@ARTICLE{barsali04,
  AUTHOR =       {Stefano Barsali and Carmine Miulli and Andrea Possenti},
  TITLE =        {A Control Strategy to Minimize Fuel Consumption of Series Hybrid Electric Vehicles},
  JOURNAL =      {IEEE Transactions on Energy Conversion},
  YEAR =         {2004},
  volume =       {19},
  number =       {1},
  pages =        {187-195},
}

@article{bauer14,
  title={Thermal and energy battery management optimization in electric vehicles using Pontryagin's maximum principle},
  author={Bauer, Sebastian and Suchaneck, Andre and Le{\'o}n, Fernando Puente},
  journal={Journal of Power Sources},
  volume={246},
  pages={808--818},
  year={2014},
  publisher={Elsevier}
}

@ARTICLE{beck97,
  AUTHOR =       {M. B. Beck and J. R. Ravetz and L. A. Mulkey and T. O. Barnwell},
  TITLE =        {On the problem of model validation for predictive exposure assessments},
  JOURNAL =      {Stochastic Hydrology and Hydraulics},
  YEAR =         {1997},
  volume =       {11},
  number =       {3},
  pages =        {229-254},
}

@ARTICLE{beck07,
  AUTHOR =       {R. Beck and A. Bollig and D. Abel},
  TITLE =        {Comparison of Two Real-Time Predictive Strategies for the Optimal Energy Management of a Hybrid Electric Vehicle},
  JOURNAL =      {Oil \& Gas Science and Technology},
  YEAR =         {2007},
  volume =       {62},
  number =       {4},
  pages =        {635-643},
}

@CONFERENCE{bedel09,
  author =       {Roger Bedell},
  title =        {Practical, 70-90{\%} Electric Bus without Overhead Wires},
  booktitle =    {EVS24},
  year =         {2009},
  address =      {Stavanger, Norway},
}

@CONFERENCE{bedel11,
  author =       {Roger Bedell and Boh Westerlund and Peter \r{A}strand},
  title =        {First Results from Field Testing of Fast Charged Hybrid Buses in {U}me\r{a}, {S}weden},
  booktitle =    {EEVC},
  year =         {2011},
  address =      {Brussels, Belgium},
}

@BOOK{bellman57,
  AUTHOR =       {Richard Bellman},
  TITLE =        {{Dynamic Programming}},
  PUBLISHER =    {Princeton Univ Pr},
  YEAR =         {1957},
  address =      {New Jersey},
}

@ARTICLE{bemporad98,
  author =       {Alberto Bemporad and Edoardo Mosca},
  title =        {Fulfilling Hard Constraints in Uncertain Linear Systems by Reference Managing},
  journal =      {Automatica},
  year =         {1998},
  volume =       {34},
  number =       {4},
  pages =        {451-461},
}

@ARTICLE{benz10,
  author =       {Michael Benz and Markus Hehn and Christopher H. Onder and Lino Guzzella},
  title =        {Model-Based Actuator Trajectories Optimization for a {D}iesel Engine Using a Direct Method},
  journal =      {J. Eng. Gas Turbines Power},
  year =         {2010},
  volume =       {133},
  number =       {3},
}

@INPROCEEDINGS{bertsekas82,
  author =       {D.P. Bertsekas and N.R. Sandell},
  title =        {Estimates of the duality gap for large-scale separable nonconvex optimization problems},
  booktitle =    {IEEE Conference on Decision and Control},
  year =         {1982},
  volume =       {21},
  pages =        {782-785},
}

@BOOK{bertsekas96,
  AUTHOR =       {Dimitri P. Bertsekas},
  TITLE =        {Constrained Optimization and Lagrange Multiplier Methods},
  PUBLISHER =    {Athena Scientific},
  YEAR =         {1996},
}

@BOOK{bertsekas00,
  AUTHOR =       {Dimitri P. Bertsekas},
  TITLE =        {{Dynamic} {Programming} and Optimal Control},
  PUBLISHER =    {Athena Scientific},
  YEAR =         {2000},
  address =      {Belmont, Massachusetts},
}

@CONFERENCE{bishu07,
  AUTHOR =       {X. Bi Shu and H. Zhixiong and M. Liu and X. Liu},
  TITLE =        {Transient modeling for heavy tracked vehicle performance and fuel consumption under accelerating conditions},
  BOOKTITLE =    {SAE World Congress},
  YEAR =         {2002},
  address =      {Detroit, Michigan},
}

@ARTICLE{bliss30,
  AUTHOR =       {Gilbert Ames Bliss},
  TITLE =        {The Problem of {Lagrange} in the Calculus of Variations},
  JOURNAL =      {American Journal of Mathematics},
  YEAR =         {1930},
  volume =       {52},
  number =       {4},
  pages =        {673-744},
}

@article{boggs95,
  title={Sequential quadratic programming},
  author={Boggs, Paul T and Tolle, Jon W},
  journal={Acta numerica},
  volume={4},
  pages={1--51},
  year={1995},
  publisher={Cambridge University Press}
}

@ARTICLE{boglietti04,
  AUTHOR =       {Aldo Boglietti and Andrea Cavagnino and Mario Lazzari and Michele Pastorelli},
  TITLE =        {International Standards for the Induction Motor Efficiency Evaluation: A Critical Analysis of the Stray-Load Loss Determination},
  JOURNAL =      {IEEE Transactions on Industry Applications},
  YEAR =         {2004},
  volume =       {40},
  number =       {5},
  pages =        {1294-1301},
}

@BOOK{boldea01,
  AUTHOR =       {Ion Boldea and Syed A. Nasar},
  TITLE =        {The Induction Machine Handbook},
  PUBLISHER =    {CRC Press},
  YEAR =         {2001},
}

@TECHREPORT{bonnet00,
  author =       {Christophe Bonnet and Hans Fritz},
  title =        {Fuel Consumption Reduction in a Platoon: Experimental Results with Two Electronically Coupled Trucks at Close Spacing},
  institution =  {SAE International},
  type =         {Technical Paper},
  year =         {2000},
  number =       {2000-01-3056},
}

@ARTICLE{borrelli05,
  AUTHOR =       {Borrelli, F. and Falcone, P. and Keviczky, T. and Asgari, J. and Hrovat, D.},
  TITLE =        {{MPC}-based approach to active steering for autonomous vehicle systems},
  JOURNAL =      {International Journal of Vehicle Autonomous Systems},
  YEAR =         {2005},
  volume =       {3},
  number =       {2},
  pages =        {265-291},
}

@BOOK{boyd04,
  AUTHOR =       {Stephen Boyd and Lieven Vandenberghe},
  TITLE =        {Convex Optimization},
  PUBLISHER =    {Cambridge University Press},
  YEAR =         {2004},
}

@ARTICLE{boyd10,
  AUTHOR =       {Stephen Boyd and Neal Parikh and Eric Chu and Borja Peleato and Jonathan Eckstein},
  TITLE =        {Distributed Optimization and Statistical Learning via the Alternating Direction Method of Multipliers},
  JOURNAL =      {Foundations and Trends in Machine Learning},
  YEAR =         {2010},
  volume =       {3},
  number =       {1},
  pages =        {1-122},
  doi =          {10.1561/2200000016},
}

@misc{buhler13,
  title={Fuel-efficient platooning of heavy duty vehicles through road topography preview information},
  author={B{\"u}hler, Lukas},
  year={2013}
}

@CONFERENCE{bradley07,
  AUTHOR =       {Thomas H. Bradley and Andrew A. Frank},
  TITLE =        {Design, demonstrations and sustainability impact assessments for plug-in hybrid electric vehicles},
  booktitle =    {Renew Sustain Energy Rev (2007)},
  YEAR =         {2007},
}

@ARTICLE{brahma12a,
  AUTHOR =       {I. Brahma and J.N. Chi},
  TITLE =        {Development of a model-based transient calibration process for {D}iesel engine electronic control module tables - {P}art 1: data requirements, processing, and analysis},
  JOURNAL =      {International Journal of Engine Research},
  YEAR =         {2012},
  volume =       {13},
  number =       {1},
  pages =        {77-96},
}

@ARTICLE{brahma12b,
  AUTHOR =       {I. Brahma and J.N. Chi},
  TITLE =        {Development of a model-based transient calibration process for {D}iesel engine electronic control module tables - {P}art 2: modelling and optimization},
  JOURNAL =      {International Journal of Engine Research},
  YEAR =         {2012},
  volume =       {13},
  number =       {2},
  pages =        {147-168},
}

@ARTICLE{brown00,
  AUTHOR =       {Phoebe R. Brown and R. Russell Rhinehart},
  TITLE =        {Demonstration of a Method for Automated Steady-State Identification in Multivariable Systems},
  JOURNAL =      {Hydrocarbon Processing},
  YEAR =         {2000},
  volume =       {79},
  number =       {9},
  pages =        {79-83},
}

@article{butcher76,
  title={On the implementation of implicit Runge-Kutta methods},
  author={Butcher, John C},
  journal={BIT Numerical Mathematics},
  volume={16},
  number={3},
  pages={237--240},
  year={1976},
  publisher={Springer}
}

@ARTICLE{bumby85,
  AUTHOR =       {J.R. Bumby and P.H. Clarke and I. Forster},
  TITLE =        {Computer modelling of the automotive energy requirements for internal combustion engine and battery electric-powered vehicles},
  JOURNAL =      {IEE proceedings},
  YEAR =         {1985},
  volume =       {132},
  number =       {5},
}

@ARTICLE{burke07,
  AUTHOR =       {Andrew F. Burke},
  TITLE =        {Batteries and Ultracapacitors for Electric, Hybrid, and Fuel Cell Vehicles},
  JOURNAL =      {Proceedings of the {IEEE}},
  YEAR =         {2007},
  volume =       {95},
  number =       {4},
  pages =        {806-820},
}

@ARTICLE{burke00,
  AUTHOR =       {Andrew F. Burke},
  TITLE =        {Ultracapacitors: why, how, and where is the technology},
  JOURNAL =      {Journal of Power Sources},
  YEAR =         {2000},
  volume =       {91},
  pages =        {37-50},
}

@ARTICLE{burke10,
  AUTHOR =       {Andrew Burke},
  TITLE =        {Ultracapacitor technologies and application in hybrid and electric vehicles},
  JOURNAL =      {International Journal of Energy Research},
  YEAR =         {2010},
  volume =       {34},
  number =       {2},
  pages =        {133-151},
}

@BOOK{bryson75,
  AUTHOR =       {Arthur E. Bryson and Yu-Chi Ho},
  TITLE =        {Applied Optimal Control},
  PUBLISHER =    {Taylor \& Francis Group},
  YEAR =         {1975},
}

% C ------------------------------------------------------------------------------------

@TECHREPORT{california01,
  INSTITUTION =  {California Air Resources Board},
  TITLE =        {Staff Paper on the Standardization of Electric Vehicle Charging Infrastructure},
  YEAR =         {2001},
}

@ARTICLE{cao95,
  AUTHOR =       {Songling Cao and R. Russell Rhinehart},
  TITLE =        {An efficient method for on-line identification of steady state},
  JOURNAL =      {J. Proc. Cont.},
  YEAR =         {1995},
  volume =       {5},
  number =       {6},
  pages =        {363-374},
}

@CONFERENCE{castro14,
  author =       {Ricardo de Castro and Mara Tanelli and Rui Esteves Ara\'ujo and Sergio M. Savaresi},
  title =        {Minimum-time Path Following in Highly Redundant Electric Vehicles},
  booktitle =    {IFAC World Congress},
  year =         {2014},
  pages  =       {3918-3923},
  address =      {Cape Town, South Africa},
}

@ARTICLE{castro16,
  author =       {Ricardo de Castro and Mara Tanelli and Rui Esteves Ara\'ujo and Sergio Matteo Savaresi},
  title =        {Minimum-Time Path-Following for Highly Redundant Electric Vehicles},
  journal =      {IEEE Transactions on Control Systems Technology},
  YEAR =         {2016},
  volume =       {24},
  number =       {2},
  pages =        {487-501},
}

@CONFERENCE{chayopitak12,
  author =       {Nattapon Chayopitak and Ruchao Pupadubsin and Santipong Karukanan and Prasit Champa},
  title =        {Design of a {1.5 kW} High Speed Switched Reluctance Motor for Electric Supercharger with Optimal Performance Assessment},
  booktitle =    {15th International Conference on Electrical Machines and Systems},
  year =         {2012},
  pages =        {1-5},
  address =      {Sapporo},
}

@TECHREPORT{chen05,
  author =       {S. Chen and O. Yanakiev},
  title =        {Transient {NOx} Emission Reduction Using Exhaust Oxygen Concentration Based Control for a {D}iesel Engine},
  institution =  {SAE International},
  type =         {Technical Paper},
  year =         {2005},
  number =       {2005-01-0372},
}

@article{chen18,
  title={Real-time predictive cruise control for eco-driving taking into account traffic constraints},
  author={Chen, Hong and Guo, Lulu and Ding, Haitao and Li, Yong and Gao, Bingzhao},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  volume={20},
  number={8},
  pages={2858--2868},
  year={2018},
  publisher={IEEE}
}

@article{chen20,
  title={Joint propulsion and cooling energy management of hybrid electric vehicles by optimal control},
  author={Chen, Boli and Li, Xuefang and Evangelou, Simos A and Lot, Roberto},
  journal={IEEE Transactions on Vehicular Technology},
  volume={69},
  number={5},
  pages={4894--4906},
  year={2020},
  publisher={IEEE}
}

@article{chen2020joint,
  title={Joint propulsion and cooling energy management of hybrid electric vehicles by optimal control},
  author={Chen, Boli and Li, Xuefang and Evangelou, Simos A and Lot, Roberto},
  journal={IEEE Transactions on Vehicular Technology},
  volume={69},
  number={5},
  pages={4894--4906},
  year={2020},
  publisher={IEEE}
}

@CONFERENCE{cole91,
  AUTHOR =       {G. H. Cole},
  TITLE =        {{SIMPLEV}: A Simple Electric Vehicle Simulation Program Version 1.0},
  YEAR =         {1991},
  publisher =    {EG and G Idaho, Inc., Idaho Falls, United States},
}

@BOOK{conejo06,
  AUTHOR =       {Antonio J. Conejo and Enrique Castillo and Roberto M�nguez and Raquel Garc�a-Bertrand},
  TITLE =        {Decomposition Techniques in Mathematical Programming. Engineering and Science Applications},
  PUBLISHER =    {Berlin/Heidelberg/New York: Springer},
  YEAR =         {2006},
}

@MISC{cones14,
  author =       {Nikolce Murgovski},
  title =        {{CONES}: {Matlab} code for convex optimization in electromobility studies},
  howpublished = {\url{https://publications.lib.chalmers.se/publication/192858}},
  year =         {2014},
}

@BOOK{conover98,
  AUTHOR =       {W. J. Conover},
  TITLE =        {Practical Nonparametric Statistics},
  PUBLISHER =    {Wiley},
  YEAR =         {1998},
  edition =      {3rd},
}

@CONFERENCE{cuddy97,
  AUTHOR =       {Matthew R. Cuddy and Keith B. Wipke},
  TITLE =        {Analysis of the Fuel Economy Benefit of Drivetrain Hybridization},
  booktitle =    {SAE International Congress \& Exposition, Detroit, Michigan},
  YEAR =         {1997},
}

@BOOK{crow60,
  AUTHOR =       {Edwin L. Crow and Frances A. Davis and Margaret W. Maxfield},
  TITLE =        {Statistics Manual},
  PUBLISHER =    {Dover Publications},
  YEAR =         {1960},
  address =      {Mineola, N.Y. 11501},
}

@MISC{cvx,
  author =       {Michael Grant and Stephen Boyd},
  title =        {{CVX}: {Matlab} Software for Disciplined Convex Programming, version 2.1},
  howpublished = {\url{http://cvxr.com/cvx}},
  year =         {2014},
}

% D ------------------------------------------------------------------------------------

@ARTICLE{delprat04,
  AUTHOR =       {Sebastien Delprat and Jimmy Lauber and Thierry Marie Guerra and J. Rimaux},
  TITLE =        {Control of a parallel hybrid powertrain: optimal control},
  JOURNAL =      {IEEE Transactions on Vehicular Technology},
  YEAR =         {2004},
  volume =       {53},
  number =       {3},
  pages =        {872-881},
}

@inproceedings{dib11,
  title={Optimal control to minimize trip time and energy consumption in electric vehicles},
  author={Dib, Wissam and Serrao, Lorenzo and Sciarretta, Antonio},
  booktitle={2011 IEEE Vehicle Power and Propulsion Conference},
  pages={1--8},
  year={2011},
  organization={IEEE}
}

@PHDTHESIS{diehl01,
  author =       {Moritz Diehl},
  title =        {Real-Time Optimization for Large Scale Nonlinear Processes},
  school =       {University of Heidelberg},
  year =         {2001},
}

@article{diehl05,
  title={A real-time iteration scheme for nonlinear optimization in optimal feedback control},
  author={Diehl, Moritz and Bock, Hans Georg and Schl{\"o}der, Johannes P},
  journal={SIAM Journal on control and optimization},
  volume={43},
  number={5},
  pages={1714--1736},
  year={2005},
  publisher={SIAM}
}

@article{ding18,
  title={On the optimal speed profile for eco-driving on curved roads},
  author={Ding, Feng and Jin, Hui},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  volume={19},
  number={12},
  pages={4000--4010},
  year={2018},
  publisher={IEEE}
}

@article{dong14,
  title={Charging infrastructure planning for promoting battery electric vehicles: An activity-based approach using multiday travel data},
  author={Dong, Jing and Liu, Changzheng and Lin, Zhenhong},
  journal={Transportation Research Part C: Emerging Technologies},
  volume={38},
  pages={44--55},
  year={2014},
  publisher={Elsevier}
}

@ARTICLE{dunbar06,
  AUTHOR =       {William B. Dunbar and Richard M. Murray},
  TITLE =        {Distributed receding horizon control for multi-vehicle formation stabilization},
  JOURNAL =      {Automatica},
  YEAR =         {2006},
  volume =       {42},
  number =       {4},
  pages =        {549-558},
}

@MANUAL{dymola10,
  TITLE =        {Dymola, dynamic modeling laboratory},
  organization = {Dynasim},
  year =         {2010},
  note =         {\url{http://www.3ds.com/products/catia/portfolio/dymola}},
}

% E ------------------------------------------------------------------------------------

@ARTICLE{ebbesen12,
  author =       {Soren Ebbesen and Philipp Elbert and Lino Guzzella},
  title =        {Battery State-of-Health Perceptive Energy Management for Hybrid Electric Vehicles},
  journal =      {IEEE Transactions On Vehicular Technology},
  year =         {2012},
  volume =       {61},
  number =       {7},
  pages =        {2893-2900},
}

@ARTICLE{ebbesen12a,
  author =       {Soren Ebbesen and Christian D\"onitz and Lino Guzzella},
  title =        {Particle swarm optimisation for hybrid electric drive-train sizing},
  journal =      {Int. J. Vehicle Design},
  year =         {2012},
  volume =       {58},
  number =       {58},
  pages =        {181-199},
}

@ARTICLE{eberle12,
  author =       {Ulrich Eberle and Bernd M\"uller and Rittmar von Helmolt},
  title =        {Fuel cell electric vehicles and hydrogen infrastructure: status 2012},
  journal =      {Energy Environ. Sci.},
  year =         {2012},
  volume =       {5},
  number =       {10},
  pages =        {8780-8798},
}

@INPROCEEDINGS{ecos,
  author={Domahidi, A. and Chu, E. and Boyd, S.},
  booktitle={European Control Conference},
  title={{ECOS}: {A}n {SOCP} solver for embedded systems},
  year={2013},
  pages={3071-3076},
}

@ARTICLE{egardt14,
  author =       {Bo Egardt and Nikolce Murgovski and Mitra Pourabdollah and Lars Johannesson},
  title =        {Electromobility Studies Based on Convex Optimization: Design and Control Issues Regarding Vehicle Electrification},
  journal =      {IEEE Control Systems Magazine},
  year =         {2014},
  volume =       {34},
  number =       {2},
  pages =        {32-49},
}

@ARTICLE{elbert13,
  AUTHOR =       {Philipp Elbert and Soren Ebbesen and Lino Guzzella},
  TITLE =        {Implementation of {D}ynamic {P}rogramming for n-Dimensional Optimal Control Problems With Final State Constraints},
  JOURNAL =      {{IEEE} Transactions on Control Systems Technology},
  year =         {2013},
  volume =       {21},
  number =       {3},
  pages =        {924-6536},
}

@ARTICLE{elbert14,
  AUTHOR =       {Philipp Elbert and Tobias N\"uesch and Andreas Ritter and Nikolce Murgovski and Lino Guzzella},
  TITLE =        {Engine On/Off Control for the Energy Management of a Serial Hybrid Electric Bus via Convex Optimization},
  JOURNAL =      {{IEEE} Transactions on Vehicular Technology},
  year =         {2014},
  volume =       {63},
  number =       {8},
  pages =        {3549-3559},
}

@CONFERENCE{elmqvist04,
  AUTHOR =       {Hilding Elmqvist and Sven Erik Mattsson and Hans Olsson and Johan Andreasson and Martin Otter and Christian Schweiger and Dag Br\"uck},
  TITLE =        {Realtime Simulation of Detailed Vehicle and Powertrain Dynamics},
  booktitle =    {SAE International},
  YEAR =         {2004},
}

@inproceedings{eriksson2016heavy,
  title={Heavy Duty Truck on Open Road--The AAC2016 Benchmark},
  author={Eriksson, Lars and Larsson, Anders and Thomasson, Andreas and Ab, Scania CV},
  booktitle={IFAC Symposium on Advances in Automotive Control},
  year={2016}
}

% F ------------------------------------------------------------------------------------

@ARTICLE{falcone08,
  AUTHOR =       {Falcone, P. and Tseng, H. E. and Borrelli, F. and Asgari, J. and Hrovat, D.},
  TITLE =        {{MPC}-based yaw and lateral stabilisation via active front steering and braking},
  JOURNAL =      {Vehicle System Dynamics: International Journal of Vehicle Mechanics and Mobility},
  year =         {2008},
  volume =       {46},
  pages =        {611-628},
}

@INPROCEEDINGS{fathy01,
  author =       {H.K. Fathy and J.A. Reyer and P.Y. Papalambros and A.G. Ulsoy},
  title =        {On the coupling between the plant and the controller optimization problems},
  booktitle =    {American Control Conference},
  year =         {2001},
  address =      {Arlington, VA},
  pages =        {1864-1869},
}

@CONFERENCE{fathy04,
  author =       {H. Fathy and P.Y. Papalambros and A.G. Ulsoy},
  title =        {On Combined Plant and Control Optimization},
  booktitle =    {8th Cairo University International Conference on Mechanical Design and Production},
  year =         {2004},
  address =      {Cairo University},
}

@INPROCEEDINGS{fellini99,
  author =       {Assanis Delagrammatikas Fellini and D. Assanis and G. Delagrammatikas and R. Fellini and Z. Filipi and J. Liedtke and N. Michelena and P. Papalambros and D. Reyes and D. Rosenbaum and A. Sales and M. Sasena},
  title =        {An Optimization Approach to Hybrid Electric Propulsion System Design},
  booktitle =    {Journal of Mechanics of Structures and Machines, Automotive Research Center Special Edition},
  year =         {1999},
  pages =        {393-421},
}

@ARTICLE{feroldi09,
  author =       {Diego Feroldi and Maria Serra and Jordi Riera},
  title =        {Design and analysis of fuel-cell hybrid systems oriented to automotive applications},
  journal =      {IEEE Transactions on Vehicular Technology},
  year =         {2009},
  volume =       {58},
  number =       {9},
  pages =        {4720-4729},
}

@ARTICLE{filipi04,
  AUTHOR =       {Z. Filipi and L. Louca and B. Daran and C-C. Lin and U. Yildir and B. Wu and M. Kokkolaras and D. Assanis and H. Peng and P. Papalambros and J. Stein and D. Szkubiel and R. Chapp},
  TITLE =        {Combined optimisation of design and power management of the hydraulic hybrid propulsion systems for the 6 x 6 medium truck},
  JOURNAL =      {International Journal of Heavy Vehicle Systems},
  YEAR =         {2004},
  volume =       {11},
  number =       {3},
  pages =        {372-402},
}

@ARTICLE{flehmig98,
  AUTHOR =       {F. Flehmig and R. v. Watzdorf and W. Marquardt},
  TITLE =        {Identification of Trends in Process Measurements using the Wavelet Transform},
  JOURNAL =      {Computers chem. Engng},
  YEAR =         {1998},
  volume =       {22},
  number =       {Supplement 1},
  pages =        {491-496},
}

@misc{FORCESPro,
  author =       {Alexander Domahidi and Juan Jerez},
  howpublished = {{embotech GmbH (\nobreak{\url{http://embotech.com/FORCES-Pro}})}},
  title =        {{FORCES Professional}},
  year =         2014,
}

@ARTICLE{fraser09,
  AUTHOR =       {Neil Fraser and Hugh Blaxill and Grant Lumsden and Mike Bassett},
  TITLE =        {Challenges for Increased Efficiency through Gasoline Engine Downsizing},
  JOURNAL =      {SAE Int. J. Engines},
  YEAR =         {2009},
  volume =       {2},
  pages =        {991-1008},
}

@CONFERENCE{fredriksson06,
  AUTHOR =       {J. Fredriksson and J. Larsson and J. Sjberg and P. Krus},
  TITLE =        {Evaluating hybrid electric and fuel cell vehicles using the {CAPSim} simulation environment},
  BOOKTITLE =    {Proceedings of the International Battery Hybrid and Fuel Cell Electric Vehicle Symposium and Exposition},
  YEAR =         {2006},
  address =      {Yokohama, Japan},
}

@article{frison20,
  title={{HPIPM}: a high-performance quadratic programming framework for model predictive control},
  author={Frison, Gianluca and Diehl, Moritz},
  journal={arXiv preprint},
  year={2020}
}

@CONFERENCE{froberg06,
  AUTHOR =       {A. Fr\"oberg},
  TITLE =        {Inverse dynamic simulation of non-quadratic {MIMO} powertrain models-application to hybrid vehicles},
  booktitle =    {Vehicle Power and Propulsion Conference (VPPC)},
  YEAR =         {2006},
}

@ARTICLE{froberg08,
  AUTHOR =       {A. Fr\"oberg and L. Nielsen},
  TITLE =        {Efficient drive cycle simulation},
  JOURNAL =      {IEEE Transactions on Vehicular Technology},
  YEAR =         {2008},
  volume =       {57},
  number =       {3},
  pages =        {1442-1453},
}

@TECHREPORT{froberg08b,
  author =       {A. Fr\"oberg and L. Nielsen},
  title =        {Optimal control utilizing analytical solutions for heavy truck cruise control},
  institution =  {Dept. of Electrical Engineering, Link\"oping University},
  year =         {2008},
  number =       {LiTH-ISY-R-2842},
  address =      {Sweden},
}

@BOOK{funck03,
  author =       {R. Funck},
  title =        {Handbook of Fuel Cells},
  publisher =    {Hoboken, NJ: Wiley},
  year =         {2003}
}

% G ------------------------------------------------------------------------------------

@TECHREPORT{gaines00,
  AUTHOR =       {Linda Gaines and Roy Cuenca},
  TITLE =        {Costs of Lithium-Ion Batteries for Vehicles},
  INSTITUTION =  {Center for Transportation Research at Argonne National Labaratory, United States Department of Energy},
  YEAR =         {2000},
  source =       {\url{http://www.doe.gov/bridge}},
}

@ARTICLE{galdi01,
  AUTHOR =       {V. Galdi and L. Ippolito and A. Piccolo and A. Vaccaro},
  TITLE =        {A genetic-based methodology for hybrid electric vehicles sizing},
  JOURNAL =      {Soft Computing - A Fusion of Foundations, Methodologies and Applications},
  YEAR =         {2001},
  volume =       {5},
  number =       {6},
  pages =        {451-457},
}

@ARTICLE{galvagno11,
  AUTHOR =       {E. Galvagno and M. Velardocchia and A. Vigliani},
  TITLE =        {Dynamic and kinematic model of a dual clutch transmission},
  JOURNAL =      {Mechanism and Machine Theory},
  YEAR =         {2011},
  volume =       {46},
  number =       {6},
  pages =        {794-805},
}

@CONFERENCE{gao12,
  AUTHOR =       {Gao, Y. and Gray, A. and Frasch, J. V. and Lin, T. and Tseng, H. E. and Hedrick, J. K. and Borrelli, F.},
  TITLE =        {Spatial predictive control for agile semi-autonomous ground vehicles},
  booktitle =    {11th International Symposium on Advanced Vehicle Control},
  YEAR =         {2012},
}

@CONFERENCE{gao09,
  AUTHOR =       {Jianping Gao and Fengchun Sun and Hongwen He and Guoming G. Zhu and Elias G. Strangas},
  TITLE =        {A Comparative Study of Supervisory Control Strategies for a Series Hybrid Electric Vehicle},
  booktitle =    {IEEE Power and Energy Engineering Conference},
  YEAR =         {2009},
}

@PHDTHESIS{gasser05,
  author =       {F. Gasser},
  title =        {An analytical, control-oriented state space model for a {PEM} fuel cell system},
  school =       {\'Ecole Polytech. F\'ed\'erale de Lausanne},
  year =         {2005},
}

@ARTICLE{gilbert95,
  author =       {Elmer G. Gilbert and Ilya Kolmanovsky and Kok Tin Tan},
  title =        {Discrete-time reference governors and the nonlinear control of systems with state and control constraints},
  journal =      {International Journal of Robust and Nonlinear Control},
  year =         {1995},
  volume =       {5},
  number =       {5},
  pages =        {487-504},
}

@PHDTHESIS{glineur01,
  AUTHOR =       {Francois Glineur},
  TITLE =        {Topics In Convex Optimization: Interior-Point Methods, Conic Duality and Approximations},
  SCHOOL =       {Mathematics and Operational Research, University of Mons, Belgium},
  YEAR =         {2001},
}

@MISC{gm,
  author =       {{General Motors}},
  title =        {{Hybrid \& electric vehicles}},
  howpublished = {\url{http://www.gm.com}},
  note =         {Accessed March 2012},
}

@TECHREPORT{grahn12,
  author =       {Markus Grahn and Krister Johansson and Christian Vartia and Tomas McKelvey},
  title =        {A structure and calibration method for data-driven modeling of {NOx} and soot emissions from a {D}iesel engine},
  institution =  {SAE International},
  type =         {Technical Paper},
  year =         {2012},
  number =       {2012-01-0355},
}

@CONFERENCE{grahn12ECOSM,
  author =       {Markus Grahn and Krister Johansson and Tomas McKelvey},
  title =        {B-splines for {D}iesel Engine Emission Modeling},
  booktitle =    {IFAC Workshop on Engine and Powertrain Control, Simulation and Modeling (ECOSM)},
  year =         {2012},
  address =      {Rueil-Malmaison, France},
}

@PHDTHESIS{grahn13,
  author =       {Markus Grahn},
  title =        {Model-based {D}iesel engine management system optimization. {A} strategy for transient engine operation},
  school =       {Chalmers University of Technology},
  year =         {2013},
  address =      {Gothenburg, Sweden},
}

@CONFERENCE{grahn13b,
  author =       {Markus Grahn and Krister Johansson and Tomas McKelvey},
  title =        {A {D}iesel Engine Management System Strategy for Transient Engine Operation},
  booktitle =    {7th IFAC Symposium on Advances in Automotive Control},
  year =         {2013},
  address =      {Tokyo, Japan},
}

@ARTICLE{grahn14a,
  author =       {Markus Grahn and Krister Johansson and Tomas McKelvey},
  title =        {Model-based diesel Engine Management System optimization for transient engine operation},
  journal =      {Control Engineering Practice},
  year =         {2014},
  volume =       {29},
  pages =        {103-114},
}

@ARTICLE{grahn14b,
  author =       {Markus Grahn and Krister Johansson and Tomas McKelvey},
  title =        {Data-driven emission model structures for diesel engine management system development},
  journal =      {International Journal of Engine Research},
  year =         {2014},
  doi =          {10.1177/1468087413512308},
}

@BOOK{grant06,
  AUTHOR =       {Michael Grant and Stephen Boyd and Y. Ye},
  TITLE =        {Global Optimization: from Theory to Implementation, Nonconvex Optimization and Its Applications},
  PUBLISHER =    {Springer},
  YEAR =         {2006},
  pages =        {155-210},
}

@INCOLLECTION{grant08,
  AUTHOR =       {Michael Grant and Stephen Boyd},
  TITLE =        {Graph implementations for nonsmooth convex programs},
  BOOKTITLE =    {Recent Advances in Learning and Control},
  PUBLISHER =    {Springer-Verlag Limited},
  YEAR =         {2008},
  editor =       {V. Blondel and S. Boyd and H. Kimura},
  series =       {Lecture Notes in Control and Information Sciences},
  pages =        {95-110},
  note =         {\url{http://stanford.edu/~boyd/graph\_dcp.html}},
}

@ARTICLE{greening01,
  AUTHOR =       {Paul Greening},
  TITLE =        {European vehicle emission legislation - present and future},
  JOURNAL =      {Topics in Catalysis},
  YEAR =         {2001},
  volume =       {16/17},
  number =       {1-4},
}

@article{guo16,
  title={Optimal energy management for {HEVs} in eco-driving applications using bi-level {MPC}},
  author={Guo, Lulu and Gao, Bingzhao and Gao, Ying and Chen, Hong},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  volume={18},
  number={8},
  pages={2153--2162},
  year={2016},
  publisher={IEEE}
}

@article{guo18,
  title={A Computationally Efficient and Hierarchical Control Strategy for Velocity Optimization of On-Road Vehicles},
  author={Guo, Lulu and Chen, Hong and Liu, Qifang and Gao, Bingzhao},
  journal={IEEE Transactions on Systems, Man, and Cybernetics: Systems},
  volume={49},
  number={1},
  pages={31--41},
  year={2018},
  publisher={IEEE}
}

@BOOK{guzzella10,
  AUTHOR =       {Lino Guzzella and Christopher H. Onder},
  TITLE =        {Introduction to Modeling and Control of Internal Combustion Engine Systems},
  PUBLISHER =    {Springer-Verlag},
  YEAR =         {2010},
}

@BOOK{guzzella13,
  AUTHOR =       {Lino Guzzella and Antonio Sciarretta},
  TITLE =        {Vehicle Propulsion Systems},
  PUBLISHER =    {Springer, Verlag},
  YEAR =         {2013},
  address =      {Berlin, Heidelberg},
  edition =      {3},
}

@BOOK{guzzella07,
  AUTHOR =       {Lino Guzzella and Antonio Sciarretta},
  TITLE =        {Vehicle Propulsion Systems, Introduction to Modeling and Optimization},
  PUBLISHER =    {Springer},
  YEAR =         {2007},
  address =      {Berlin, Heidelberg},
  edition =      {2nd},
}

@ARTICLE{guzzella99,
  AUTHOR =       {Lino Guzzella and Alois Amstutz},
  TITLE =        {{CAE} Tools for Quasi-Static Modeling and Optimization of Hybrid Powertrains},
  JOURNAL =      {IEEE Transactions on Vehicular Technology},
  YEAR =         {1999},
  volume =       {48},
  number =       {6},
}

% H ------------------------------------------------------------------------------------

@article{hamednia18,
  title={Predictive velocity control in a hilly terrain over a long look-ahead horizon},
  author={Hamednia, Ahad and Murgovski, Nikolce and Fredriksson, Jonas},
  journal={IFAC-PapersOnLine},
  volume={51},
  number={31},
  pages={485--492},
  year={2018},
  publisher={Elsevier}
}

@CONFERENCE{hamedniaitsc20,
  author =       {Ahad Hamednia and Nikolce Murgovski and Jonas Fredriksson},
  title =        {Time optimal and eco-driving mission planning under traffic constraints},
  booktitle =    {Intelligent Transportation Systems (ITSC)},
  year =         {2020},
  address =      {Rhodos, Greece},
}

@article{hamednia21,
  title={Computationally efficient algorithm for eco-driving over long look-ahead horizons},
  author={Hamednia, Ahad and Sharma, Nalin Kumar and Murgovski, Nikolce and Fredriksson, Jonas},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  year={2021},
  publisher={IEEE}
}

@inproceedings{hamedniaitsc21,
  title={Electric Vehicle Eco-driving under Wind Uncertainty},
  author={Hamednia, Ahad and Razi, Maryam and Murgovski, Nikolce and Fredriksson, Jonas},
  booktitle={2021 IEEE International Intelligent Transportation Systems Conference (ITSC)},
  pages={3502--3508},
  year={2021},
  organization={IEEE}
}

@ARTICLE{hamilton34,
  AUTHOR =       {William Rowan Hamilton},
  TITLE =        {On a general method in dynamics},
  JOURNAL =      {Philosophical Transactions of the Royal Society},
  YEAR =         {1834},
  volume =       {2},
  pages =        {247-308},
}

@ARTICLE{hamilton35,
  AUTHOR =       {William Rowan Hamilton},
  TITLE =        {Second essay on a general method in dynamics},
  JOURNAL =      {Philosophical Transactions of the Royal Society},
  YEAR =         {1835},
  volume =       {1},
  pages =        {95-144},
}

@article{hannan2018,
  title={State-of-the-art and energy management system of lithium-ion batteries in electric vehicle applications: Issues and recommendations},
  author={Hannan, Mahammad A and Hoque, Md Murshadul and Hussain, Aini and Yusof, Yushaizad and Ker, Pin Jern},
  journal={Ieee Access},
  volume={6},
  pages={19362--19378},
  year={2018},
  publisher={IEEE}
}

@misc{hanson17,
  title={Systems and methods for multi-mode unmanned vehicle mission planning and control},
  author={Hanson, Bruce Becker and Hanson, Thomas Edward},
  year={2017},
  month=jun # "~6",
  publisher={Google Patents},
  note={US Patent 9,669,904}
}

@article{hartl95,
  title={A survey of the maximum principles for optimal control problems with state constraints},
  author={Hartl, Richard F and Sethi, Suresh P and Vickson, Raymond G},
  journal={SIAM review},
  volume={37},
  number={2},
  pages={181--218},
  year={1995},
  publisher={SIAM}
}

@ARTICLE{hawkins12,
  AUTHOR =       {Troy R. Hawkins and Ola Moa Gausen and Anders Hammer Str{\o}mman},
  TITLE =        {Environmental impacts of hybrid and electric vehicles---a review},
  JOURNAL =      {The International Journal of Life Cycle Assessment},
  YEAR =         {2012},
  volume =       {17},
  number =       {8},
  pages =        {997-1014},
}

@CONFERENCE{hayat03,
  AUTHOR =       {O. Hayat and M. Lebrun and E. Domingues},
  TITLE =        {Powertrain drivability evaluation: Analysis and simplification of dynamic models},
  BOOKTITLE =    {SAE World Congress},
  YEAR =         {2003},
  address =      {Detroit, Michigan},
}

@article{he16,
  title={Fuel consumption optimization of heavy-duty vehicles with grade, wind, and traffic information},
  author={He, Chaozhe R and Maurer, Helmut and Orosz, G{\'a}bor},
  journal={Journal of Computational and Nonlinear Dynamics},
  volume={11},
  number={6},
  year={2016},
  publisher={American Society of Mechanical Engineers Digital Collection}
}

@BOOK{heisler02,
  AUTHOR =       {Heinz Heisler},
  TITLE =        {Advanced Vehicle Technology},
  PUBLISHER =    {A Butterworth-Heinemann Title},
  YEAR =         {2002},
  edition =      {2nd},
  address =      {Linacre House, Jordan Hill, Oxford},
}

@article{held18,
  title={Optimal Speed Control of a Heavy-Duty Vehicle in Urban Driving},
  author={Held, Manne and Fl{\"a}rdh, Oscar and M{\aa}rtensson, Jonas},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  volume={20},
  number={4},
  pages={1562--1573},
  year={2018},
  publisher={IEEE}
}

@phdthesis{held20,
  title={Fuel-Efficient Look-Ahead Control for Heavy-Duty Vehicles with Varying Velocity Demands},
  author={Held, Manne},
  year={2020},
  school={KTH Royal Institute of Technology}
}

@ARTICLE{hellstrom09,
  author =       {Erik Hellstr\"om and Maria Ivarsson and Jan \r{A}slund and Lars Nielsen},
  title =        {Look-ahead control for heavy trucks to minimize trip time and fuel consumption},
  journal =      {Control Engineering Practice},
  year =         {2009},
  volume =       {17},
  number =       {2},
  pages =        {245-254},
}

@ARTICLE{hellstrom10,
  author =       {Erik Hellstr\"om and Jan \r{A}slund and Lars Nielsen},
  title =        {Design of an efficient algorithm for fuel-optimal look-ahead control},
  journal =      {Control Engineering Practice},
  year =         {2010},
  volume =       {18},
  number =       {11},
  pages =        {1318-1327},
}

@article{hellstrom10b,
  author	= {Erik Hellstr{\"o}m and Jan \r{A}slund and Lars Nielsen},
  title		= {Management of Kinetic and Electric Energy in Heavy Trucks},
  journal	= {SAE International Journal of Engines},
  year		= {2010},
  volume	= {3},
  number	= {1},
  pages		= {1152-1163},
}

@ARTICLE{heppeler16a,
  AUTHOR =       {Gunter Heppeler and Marcus Sonntag and Uli Wohlhaupter and Oliver Sawodny},
  TITLE =        {Predictive planning of optimal velocity and state of charge trajectories for hybrid electric vehicles},
  JOURNAL =      {Control Engineering Practice},
  YEAR =         {2016},
  volume =       {61},
  pages =        {229-243},
}

@BOOK{heywood88,
  AUTHOR =       {John B. Heywood},
  TITLE =        {Internal Combustion Engine Fundamentals},
  PUBLISHER =    {McGraw-Hill},
  YEAR =         {1988},
}

@BOOK{hiereth07,
  author =       {Hermann Hiereth and Peter Prenninger},
  title =        {Charging the Internal Combustion Engine},
  publisher =    {Springer},
  year =         {2007},
}

@PHDTHESIS{hofman_thesis,
  AUTHOR =       {Theo Hofman},
  TITLE =        {Framework for combined control and design optimization of hybrid vehicle propulsion systems},
  SCHOOL =       {Eindhoven University of Technology},
  YEAR =         {2007},
}

@ARTICLE{hofman07,
  AUTHOR =       {T. Hofman and M. Steinbuch and R.M. van Druten and A.F.A. Serrarens},
  TITLE =        {Parametric Modeling of Components for Selection and Specification of Hybrid Vehicle Drivetrains},
  JOURNAL =      {WEVA Journal},
  YEAR =         {2007},
  volume =       {1},
  number =       {1},
  pages =        {215-224},
}

@ARTICLE{hofman08,
  AUTHOR =       {T. Hofman and M. Steinbuch and R.M. van Druten and A.F.A. Serrarens},
  TITLE =        {Hybrid component specification optimisation for a medium-duty hybrid electric truck},
  JOURNAL =      {Int. J. Heavy Vehicle Systems},
  YEAR =         {2008},
  volume =       {15},
  number =       {2/3/4},
  pages =        {256-392},
}

@CONFERENCE{holder06,
  AUTHOR =       {Courtney Holder and James Gover},
  TITLE =        {Optimizing the Hybridization Factor for a Parallel Hybrid Electric Small Car},
  booktitle =    {IEEE Vehicle Power and Propulsion Conference (VPPC)},
  YEAR =         {2006},
}

@MISC{honda,
  author =       {{Honda Motor Corporation}},
  title =        {{Honda Civic Hybrid} and {Honda Insight}},
  howpublished = {\url{http://honda.com}},
  note =         {Accessed March 2012},
}

@ARTICLE{horiba05,
  AUTHOR =       {T. Horiba and T. Maeshima and T. Matsumura and M. Koseki and J. Arai and Y. Muranaka},
  TITLE =        {Applications of high power density lithium ion batteries},
  JOURNAL =      {Journal of Power Sources},
  YEAR =         {2005},
  volume =       {146},
  pages =        {107-110},
}

@ARTICLE{hotelling31,
  AUTHOR =       {Harold Hotelling},
  TITLE =        {The Generalization of Student's Ratio},
  JOURNAL =      {Ann. Math. Statist.},
  YEAR =         {1931},
  volume =       {2},
  number =       {3},
  pages =        {360-378},
}

@ARTICLE{hovgard18,
  AUTHOR =       {Mattias Hovgard and Oscar Jonsson and Nikolce Murgovski and Martin Sanfridson and Jonas Fredriksson},
  TITLE =        {Cooperative energy management of electrified vehicles on hilly roads},
  JOURNAL =      {Control Engineering Practice},
  YEAR =         {2018},
  volume =       {73},
  pages =        {66-78},
}

@CONFERENCE{hu04,
  AUTHOR =       {Xiaolin Hu and Zhongfan Wang and Lianying Liao},
  TITLE =        {Multi-Objective Optimization of {HEV} Fuel Economy and Emissions Using Evolutionary Computation},
  booktitle =    {SAE World Congress Detroit, Michigan},
  YEAR =         {2004},
}

@ARTICLE{hu13,
  AUTHOR =       {Xiaosong Hu and Nikolce Murgovski and Lars Johannesson and Bo Egardt},
  TITLE =        {Energy efficiency analysis of a series plug-in hybrid electric bus with different energy management strategies and battery sizes},
  JOURNAL =      {Applied Energy},
  YEAR =         {2013},
  volume =       {111},
  number =       {0},
  pages =        {1001-1009},
}

@ARTICLE{hu14a,
  AUTHOR =       {Xiaosong Hu and Nikolce Murgovski and Lars Johannesson and Bo Egardt},
  TITLE =        {Comparison of Three Electrochemical Energy Buffers Applied to a Hybrid Bus Powertrain with Simultaneous Optimal Sizing and Energy Management},
  JOURNAL =      {IEEE Transactions on Intelligent Transportation Systems},
  YEAR =         {2014},
  volume =       {15},
  number =       {3},
  pages =        {1193-1205},
}

@ARTICLE{hu15a,
  AUTHOR =       {Xiaosong Hu and Nikolce Murgovski and Lars Johannesson and Bo Egardt},
  TITLE =        {Optimal dimensioning and power management of a fuel cell/battery hybrid bus via convex programming},
  JOURNAL =      {IEEE/ASME Transactions on Mechatronics},
  YEAR =         {2015},
  volume =       {20},
  number =       {1},
  pages =        {457-468},
}

@ARTICLE{hu15b,
  AUTHOR =       {Xiaosong Hu and Lars Johannesson and Nikolce Murgovski and Bo Egardt},
  TITLE =        {Longevity-conscious dimensioning and power management of the hybrid energy storage system for a fuel cell hybrid electric bus},
  JOURNAL =      {Applied Energy},
  YEAR =         {2015},
  volume =       {137},
  pages =        {913-924},
}

@BOOK{hucho87,
  editor =       {Wolf-Heinrich Hucho},
  title =        {Aerodynamics of Road Vehicles},
  publisher =    {Butterworth-Heinemann},
  year =         {1987},
  edition =      {4},
  isbn =         {978-0-7506-1267-8},
}

@TECHREPORT{hultebeg09,
  author =       {Christian Hulteberg and Diane Aagesen},
  title =        {Hydrogen Production for Refueling Applications},
  institution =  {Swedish Gas Centre (SGC)},
  year =         {2009},
  number =       {SGC-R-210-SE},
}

% I ------------------------------------------------------------------------------------

@MISC{IEEE91,
  author =       {{IEEE std 112-1991}},
  title =        {{IEEE} standard test procedure for polyphase induction motors and generators},
  howpublished = {Institute of Electrical and Electronics Engineers},
  year =         {1991},
}

@TECHREPORT{icct13,
  author =       {{ICCT}},
  title =        {World-Harmonized Light-Duty Vehicles Test Procedure {(WLTP)}},
  institution =  {International Council on Clean Transportation},
  year =         {2013},
}

% J ------------------------------------------------------------------------------------
@article{jaguemont15,
  title={Lithium-ion battery aging experiments at subzero temperatures and model development for capacity fade estimation},
  author={Jaguemont, Joris and Boulon, Lo{\"\i}c and Venet, Pascal and Dub{\'e}, Yves and Sari, Ali},
  journal={IEEE Transactions on Vehicular Technology},
  volume={65},
  number={6},
  pages={4328--4343},
  year={2015},
  publisher={IEEE}
}

@article{jaguemont16,
  title={Thermal management of a hybrid electric vehicle in cold weather},
  author={Jaguemont, Joris and Boulon, Loic and Dube, Yves and Martel, Francois},
  journal={IEEE Transactions on Energy Conversion},
  volume={31},
  number={3},
  pages={1110--1120},
  year={2016},
  publisher={IEEE}
}

@MASTERSTHESIS{jeber15,
  author =       {Mandus Jeber},
  title =        {Fuel efficient control of vehicle platoons using road topography information},
  school =       {Chalmers University of Technology},
  year =         {2015},
  address =      {Gothenburg, Sweden},
}

@phdthesis{jeffs19,
  title={An Investigation Into the Optimal Operation of a Complex Heat Pump for the Complete Thermal Management of an Electric Vehicle in Cold Climates},
  author={Jeffs, James},
  year={2019},
  school={University of Warwick}
}

@ARTICLE{jiang03,
  AUTHOR =       {Taiwen Jiang and Bingzhen Chen and Xiaorong He and Paul Stuart},
  TITLE =        {Application of steady-state detection method based on wavelet transform},
  JOURNAL =      {Computers and Chemical Engineering},
  YEAR =         {2003},
  pages =        {569-578},
  volume =       {27},
}

@CONFERENCE{jinming08,
  AUTHOR =       {Jinming Liu and Huei Peng},
  TITLE =        {Automated Modelling of Power-Split Hybrid Vehicles},
  BOOKTITLE =    {Proceedings of the World Congress The International Federation of Automatic Control},
  YEAR =         {2008},
  address =      {Seoul, Korea},
}

@ARTICLE{johannesson05,
  AUTHOR =       {Lars Johannesson and Mattias \r{A}sbog\r{a}rd and Bo Egardt},
  TITLE =        {Assessing the Potential of Predictive Control for Hybrid Vehicle Powertrains using Stochastic {Dynamic} {Programming}},
  JOURNAL =      {IEEE Transactions on Intelligent Transportation Systems},
  YEAR =         {2007},
  volume =       {8},
  number =       {1},
  pages =        {71-83},
}

@ARTICLE{johannesson09a,
  AUTHOR =       {Lars Johannesson and Stefan Pettersson and Bo Egardt},
  TITLE =        {Predictive energy management of a {4QT} series-parallel hybrid electric bus},
  JOURNAL =      {Control Engineering Practice},
  YEAR =         {2009},
  volume =       {17},
  number =       {12},
  pages =        {1440-1453},
}

@PHDTHESIS{johannesson09,
  AUTHOR =       {Lars Johannesson},
  TITLE =        {Predictive Control of Hybrid Electric Vehicles on Prescribed Routes},
  SCHOOL =       {Chalmers University of Technology},
  YEAR =         {2009},
  address =      {G\"oteborg, Sweden},
}

@CONFERENCE{johannesson13,
  author =       {Lars Johannesson and Nikolce Murgovski and Soren Ebbessen and Bo Egardt and Esteban Gelso and Jonas Hellgren},
  title =        {Including a Battery State of Health model in the {HEV} component sizing and optimal control problem},
  booktitle =    {IFAC Symposium on Advances in Automotive Control},
  year =         {2013},
  address =      {Tokyo, Japan},
}

@ARTICLE{johannesson15a,
  author =       {Lars Johannesson and Nikolce Murgovski and Erik Jonasson and Jonas Hellgren and Bo Egardt},
  title =        {Predictive energy management of hybrid long-haul trucks},
  journal =      {Control Engineering Practice},
  year =         {2015},
  volume =       {41},
  pages =        {83-97},
}

@CONFERENCE{johannesson15b,
  author =       {Lars Johannesson and Magnus Nilsson and Nikolce Murgovski},
  title =        {Look-ahead vehicle energy management with traffic predictions},
  booktitle =    {IFAC Workshop on Engine and Powertrain Control, Simulation and Modeling (E-COSM)},
  year =         {2015},
  address =      {Columbus, Ohio, USA},
  volume =       {48},
  issue =       {15},
  pages =        {244-251},
}

@MASTERSTHESIS{johansson11,
  AUTHOR =       {Michael Johansson and Oscar Olsson},
  TITLE =        {Feasibility study of dual-mode buses in {G}othenburg's public transport},
  SCHOOL =       {Chalmers University of Technology, Gothenburg, Sweden},
  YEAR =         {2011},
}

@ARTICLE{johnson13,
  AUTHOR =       {Timothy V. Johnson},
  TITLE =        {Vehicular Emissions in Review},
  JOURNAL =      {SAE Int. J. Engines},
  YEAR =         {2013},
  volume =       {5},
  number =       {2},
  pages =        {216-234},
  publisher =    {SAE International},
}

% K ------------------------------------------------------------------------------------

@CONFERENCE{kachapornkul12,
  AUTHOR =       {Seubsuang Kachapornkul and Pakasit Somsiri and Ruchao Pupadubsin and Niyom Nulek},
  TITLE =        {Low Cost High Speed Switched Reluctance Motor Drive for Supercharger Applications},
  BOOKTITLE =    {15th International Conference on Electrical Machines and Systems},
  YEAR =         {2012},
  address =      {Sapporo},
  pages =        {1-6},
}

@TECHREPORT{kaist09,
  TITLE =        {On-line electric vehicle},
  INSTITUTION =  {Korea Advanced Institute of Science and Technology ({KAIST})},
  YEAR =         {2009},
}

@ARTICLE{kamal11,
  title={Ecological vehicle control on roads with up-down slopes},
  author={Kamal, Md Abdus Samad and Mukai, Masakazu and Murata, Junichi and Kawabe, Taketoshi},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  volume={12},
  number={3},
  pages={783--794},
  year={2011},
  publisher={IEEE}
}

@article{kamal12,
  title={Model predictive control of vehicles on urban roads for improved fuel economy},
  author={Kamal, Md Abdus Samad and Mukai, Masakazu and Murata, Junichi and Kawabe, Taketoshi},
  journal={IEEE Transactions on control systems technology},
  volume={21},
  number={3},
  pages={831--841},
  year={2012},
  publisher={IEEE}
}

@CONFERENCE{kang99,
  AUTHOR =       {{Jun-Mo} Kang and Ilya Kolmanovsky and J.W. Grizzle},
  TITLE =        {Approximate dynamic programming solutions for lean burn engine aftertreatment},
  BOOKTITLE =    {Proceedings of the IEEE Conference on Decision and Control},
  YEAR =         {1999},
  volume =       {2},
  pages =        {1703-1708},
}

@ARTICLE{kang01,
  AUTHOR =       {{Jun-Mo} Kang and Ilya Kolmanovsky and J.W. Grizzle},
  TITLE =        {Dynamic Optimization of Lean Burn Engine Aftertreatment},
  JOURNAL =      {Journal of Dynamic Systems, Measurement and Control},
  YEAR =         {2001},
  volume =       {123},
  number =       {2},
  pages =        {153-160},
}

@ARTICLE{karen99,
  AUTHOR =       {Karen L. Butler and Mehrdad Ehsani and Preyas Kamath},
  TITLE =        {A {Matlab}-Based Modeling and Simulation Package for Electric and Hybrid Electric Vehicle Design},
  JOURNAL =      {IEEE Transactions on Vehicular Technology},
  YEAR =         {1999},
  volume =       {48},
  number =       {6},
}

@ARTICLE{katrasnik07,
  AUTHOR =       {Toma\v{z} Katra\v{s}nik and Ferdinand Trenc and Samuel Rodman Opre\v{s}nik},
  TITLE =        {Analysis of Energy Conversion Efficiency in Parallel and Series Hybrid Powertrains},
  JOURNAL =      {IEEE Transactions on Vehicular Technology},
  YEAR =         {2007},
  volume =       {56},
  number =       {6},
  pages =        {3649-3659},
}

@ARTICLE{katrasnik10,
  AUTHOR =       {Toma\v{z} Katra\v{s}nik},
  TITLE =        {Analytical method to evaluate fuel consumption of hybrid electric vehicles at balanced energy content of the electric storage devices},
  JOURNAL =      {Applied Energy},
  YEAR =         {2010},
  volume =       {87},
  pages =        {3330-3339},
}

@BOOK{kaviany01,
  AUTHOR =       {Massoud Kaviany},
  TITLE =        {Principles of Heat Transfer},
  PUBLISHER =    {Wiley-Interscience},
  YEAR =         {2001},
}

@MASTERSTHESIS{kemppainen12,
  author =       {Josefin Kemppainen},
  title =        {Model Predictive Control for Heavy Duty Vehicle Platooning},
  school =       {Link\"oping University},
  year =         {2012},
  address =      {Link\"oping, Sweden},
}

@CONFERENCE{keulen10,
  author =       {Thijs van Keulen and Bram de Jager and Darren Foster and Maarten Steinbuch},
  title =        {Velocity trajectory optimization in hybrid electric trucks},
  booktitle =    {American Control Conference},
  year =         {2010},
  pages  =       {5074-5079},
  address =      {Marriott Waterfront, Baltimore, MD, USA},
}

@CONFERENCE{keulen11,
  author =       {Thijs van Keulen and Bram de Jager and Maarten Steinbuch},
  title =        {Optimal Trajectories for Vehicles with Energy Recovery Options},
  booktitle =    {IFAC World Congress},
  year =         {2011},
  pages  =       {3831-3836},
  address =      {Milan, Italy},
}

@ARTICLE{Keulen14,
  AUTHOR =       {Thijs van Keulen and Jan Gillot and Bram de Jager and Maarten Steinbuch},
  TITLE =        {Solution for state constrained optimal control problems applied to
power split control for hybrid vehicles},
  JOURNAL =      {Automatica},
  YEAR =         {2014},
  volume =       {50},
  number =       {1},
  pages =        {187-192},
}


@ARTICLE{khayyam11,
  AUTHOR =       {Hamid Khayyam and Abbas Z. Kouzani and Eric J. Hu and Saeid Nahavandi},
  TITLE =        {Coordinated energy management of vehicle air conditioning system},
  JOURNAL =      {Applied Thermal Engineering},
  YEAR =         {2011},
  volume =       {31},
  number =       {5},
  pages =        {750-764},
}

@CONFERENCE{kim06,
  AUTHOR =       {{Min-Joong} Kim and Huei Peng},
  TITLE =        {Combined Control/Plant Optimization of Fuel Cell Hybrid Vehicles},
  booktitle =    {Proceedings of the American Control Conference Minneapolis, Minnesota, USA},
  YEAR =         {2006},
}

@ARTICLE{kim07,
  AUTHOR =       {{Min-Joong} Kim and Huei Peng},
  TITLE =        {Power management and design optimization of fuel cell/battery hybrid vehicles},
  JOURNAL =      {Journal of Power Sources},
  YEAR =         {2007},
  volume =       {165},
  number =       {2},
  pages =        {819-832},
}

@CONFERENCE{kirches13,
  author =       {Christian Kirches and Hans Georg Bock and Johannes P. Schl\"oder and Sebastian Sager},
  title =        {Mixed-integer {NMPC} for predictive cruise control of heavy-duty trucks},
  booktitle =    {European Control Conference},
  year =         {2013},
  pages  =       {4118-4123},
  address =      {Z\"urich, Switzerland},
}

@BOOK{kirsch64,
  AUTHOR =       {David A. Kirsch},
  TITLE =        {The Electric Vehicle and the Burden of History},
  PUBLISHER =    {Rutgers University Press},
  YEAR =         {1964},
}

@TECHREPORT{koegler01,
  author =       {Hans-Michael Koegler and Alois Fuerhapter and Monika Mayer and Kurt Gschweitl},
  title =        {{DGI}-Engine Calibration, Using New Methodology with {CAMEO}},
  institution =  {SAE International},
  type =         {Technical Paper},
  year =         {2001},
  number =       {2001-24-0012},
}

@ARTICLE{kohler02,
  AUTHOR =       {U. K\"ohler and J. K\"umpers and M. Ullrich},
  TITLE =        {High performance nickel-metal hydride and lithium-ion batteries},
  JOURNAL =      {Journal of Power Sources},
  YEAR =         {2002},
  volume =       {105},
  pages =        {139-144},
}

@CONFERENCE{kolmanovsky99,
  AUTHOR =       {Ilya Kolmanovsky and Michiel van Nieuwstadt and Jing Sun},
  TITLE =        {Optimization of Complex Powertrain Systems for Fuel Economy and Emissions},
  BOOKTITLE =    {Proceedings of the IEEE International Conference on Control Applications},
  YEAR =         {1999},
  address =      {Kohala Coast-Island of Hawai, USA},
}

@CONFERENCE{kolmanovsky02,
  AUTHOR =       {Ilya Kolmanovsky and Irina Siverguina and Bob Lygoe},
  TITLE =        {Optimization of Powertrain Operating Policy for Feasibility Assessment and Calibration: Stochastic {Dynamic} {Programming} Approach},
  BOOKTITLE =    {Proceedings of the American Control Conference},
  YEAR =         {2002},
  address =      {Anchorage, AK},
}

@CONFERENCE{kolmanovsky05,
  AUTHOR =       {Ilya V. Kolmanovsky and Shiva N. Sivashankar and Jing Sun},
  TITLE =        {Optimal control-based powertrain feasibility assessment: A software implementation perspective},
  BOOKTITLE =    {American Control Conference},
  YEAR =         {2005},
  address =      {Portland, {OR}, USA},
}

@ARTICLE{koot05,
  AUTHOR =       {Michiel Koot and J. T. B. A. Kessels and Bram de Jager and W. P. M. H. Heemels and P. P. J. van den Bosch and Maarten Steinbuch},
  TITLE =        {Energy Management Strategies for Vehicular Electric Power Systems},
  JOURNAL =      {IEEE Transactions on Vehicular Technology},
  YEAR =         {2005},
  volume =       {54},
  number =       {3},
  pages =        {771-782},
}

@ARTICLE{kraytsberg11,
  AUTHOR =       {Alexander Kraytsberg and Yair {Ein-Eli}},
  TITLE =        {Review on {Li}-air batteries - {Opportunities}, limitations and perspective},
  JOURNAL =      {Journal of Power Sources},
  YEAR =         {2011},
  volume =       {196},
  number =       {3},
  pages =        {886-893},
}

@INPROCEEDINGS{kuwata08,
  author =       {Kuwata, Y. and Fiore, G.A. and Teo, J. and Frazzoli, E. and How, J.P.},
  title =        {Motion planning for urban driving using {RRT}},
  booktitle =    {IEEE/RSJ International Conference on Intelligent Robots and Systems},
  year =         {2008},
  pages =        {1681-1686},
}

% L ------------------------------------------------------------------------------------
@article{lajunen12,
  title={Evaluation of energy storage system requirements for hybrid mining loaders},
  author={Lajunen, Antti and Suomela, Jussi},
  journal={IEEE transactions on vehicular technology},
  volume={61},
  number={8},
  pages={3387--3393},
  year={2012},
  publisher={IEEE}
}

@BOOK{larminie03,
  AUTHOR =       {James Larminie and John Lowry},
  TITLE =        {Electric Vehicle Technology Explained},
  PUBLISHER =    {John Wiley \& Sons Ltd.},
  YEAR =         {2003},
}

@CONFERENCE{larsson12,
  AUTHOR =       {Viktor Larsson and Lars Johannesson and Bo Egardt and Anders Lassson},
  TITLE =        {Benefit of route recognition in energy management of plug-in hybrid electric vehicles},
  BOOKTITLE =    {Proceeding of the American Control Conference},
  YEAR =         {2012},
}

@BOOK{law99,
  AUTHOR =       {Averill M. Law and W. David Kelton},
  TITLE =        {Simulation Modeling and Analysis},
  PUBLISHER =    {McGraw-Hill},
  YEAR =         {1999},
  edition =      {3rd},
}

@article{leduc03,
  author =       {P. Leduc and B. Dubar and A. Ranini and G. Monnier},
  journal =      {Oil \& Gas Science and Technology},
  number =       {1},
  pages =        {115-127},
  title =        {Downsizing of Gasoline Engine: an Efficient Way to Reduce {CO2} Emissions},
  volume =       {58},
  year =         {2003},
}

@ARTICLE{lei03,
  AUTHOR =       {Lei Ma and Masayuki Sanada and Shigeo Morimoto and Yoji Takeda},
  TITLE =        {Prediction of Iron Loss in Rotating Machines With Rotational Loss Included},
  JOURNAL =      {IEEE Transactions on Magnetics},
  YEAR =         {2003},
  volume =       {39},
  number =       {4},
  pages =        {2036-2041},
}

@ARTICLE{levine66,
  author =       {W. S. Levine and M. Athans},
  title =        {On the optimal error regulation of a string of moving vehicles},
  journal =      {IEEE Transactions on Automatic Control},
  year =         {1966},
  volume =       {11},
  number =       {3},
  pages =        {355-361},
}

@CONFERENCE{liang11,
  author =       {Kuo-Yun Liang and Assad Alam and Ather Gattami},
  title =        {The Impact of Heterogeneity and Order in Heavy Duty Vehicle Platooning Networks},
  booktitle =    {IEEE Vehicular Networking Conference (VNC)},
  year =         {2011},
  address =      {Amsterdam, The Netherlands},
  pages =        {291-297},
}

@ARTICLE{liang16,
  AUTHOR =       {Kuo-Yun Liang and Jonas M\r{a}rtensson and Karl H. Johansson},
  TITLE =        {Heavy-duty vehicle platoon formation for fuel efficiency},
  JOURNAL =      {IEEE Transactions on Intelligent Transportation Systems},
  YEAR =         {2016},
  volume =       {17},
  number =       {4},
  pages =        {1051-1061},
}

@article{limb18,
  title={Economic viability and environmental impact of in-motion wireless power transfer},
  author={Limb, Braden J and Asher, Zachary D and Bradley, Thomas H and Sproul, Evan and Trinko, David A and Crabb, Benjamin and Zane, Regan and Quinn, Jason C},
  journal={IEEE Transactions on Transportation Electrification},
  volume={5},
  number={1},
  pages={135--146},
  year={2018},
  publisher={IEEE}
}

@ARTICLE{lin03,
  AUTHOR =       {{Chan-Chiao} Lin and Huei Peng and Jessy W. Grizzle and {Jun-Mo} Kang},
  TITLE =        {Power Management Strategy for a Parallel Hybrid Electric Truck},
  JOURNAL =      {IEEE Transactions on Control Systems Technology},
  YEAR =         {2003},
  volume =       {11},
  number =       {6},
  pages =        {839-849},
}

@CONFERENCE{lin04,
  AUTHOR =       {{Chan-Chiao} Lin and Huei Peng and Jessy W. Grizzle},
  TITLE =        {A Stochastic Control Strategy for Hybrid Electric Vehicles},
  BOOKTITLE =    {Proceeding of the American Control Conference},
  YEAR =         {2004},
}

@ARTICLE{lin04a,
  AUTHOR =       {D. Lin and P. Zhou and W. N. Fu and Z. Badics and Z. J. Cendes},
  TITLE =        {A Dynamic Core Loss Model for Soft Ferromagnetic and Power Ferrite Materials in Transient Finite Element Analysis},
  JOURNAL =      {IEEE Transactions on Magnetics},
  YEAR =         {2004},
  volume =       {40},
  number =       {2},
  pages =        {1318-1321},
}

@ARTICLE{lindgarde15,
  author =       {Olof Lindg\"arde and Lei Feng and Anders Tenstam and Mikael Soderman},
  title =        {Optimal Vehicle Control for Fuel Efficiency},
  journal =      {SAE International Journal of Commercial Vehicles},
  year =         {2015},
  volume =       {8},
  number =       {2},
  pages =        {682-694},
}

@article{lindgarde16,
  title={Optimal complete vehicle control for fuel efficiency},
  author={Lindg{\"a}rde, Olof and S{\"o}derman, Mikael and Tenstam, Anders and Feng, Lei},
  journal={Transportation Research Procedia},
  volume={14},
  pages={1087--1096},
  year={2016},
  publisher={Elsevier}
}

@CONFERENCE{linming08,
  AUTHOR =       {Jinming Liu and Huei Peng},
  TITLE =        {Automated Modelling of Power-Split Hybrid Vehicles},
  BOOKTITLE =    {Proceedings of the World Congress The International Federation of Automatic Control},
  YEAR =         {2008},
  address =      {Seoul, Korea},
}

@ARTICLE{lipp14,
  AUTHOR =       {Thomas Lipp and Stephen Boyd},
  TITLE =        {Minimum-Time Speed Optimization Along a Fixed Path},
  JOURNAL =      {International Journal of Control},
  YEAR =         {2014},
  volume =       {87},
  number =       {6},
  pages =        {1297-1311},
}

@BOOK{ljung99,
  AUTHOR =       {Lennart Ljung},
  TITLE =        {System Identification: Theory for the User},
  PUBLISHER =    {Prentice Hall PTR},
  YEAR =         {1999},
  edition =      {2nd},
}

@MISC{lofberg04,
  author =       {Johan L\"ofberg},
  title =        {{YALMIP}: A Toolbox for Modeling and Optimization in {Matlab}},
  howpublished = {In Proceedings of the CACSD Conference, Taipei, Taiwan, \url{http://users.isy.liu.se/johanl/yalmip}},
  year =         {2004},
}

@MISC{lohner,
  author =       {{Jacob Lohner \& Co}},
  title =        {The First Hybrid Vehicle},
  howpublished = {\url{http://www.hybrid-vehicle.org}},
  note =         {Accessed March 2012},
}

\RequirePackage{filecontents}


@ARTICLE{luo15,
  title={Intelligent hybrid electric vehicle ACC with coordinated control of tracking ability, fuel economy, and ride comfort},
  author={Luo, Yugong and Chen, Tao and Zhang, Shuwei and Li, Keqiang},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  volume={16},
  number={4},
  pages={2303--2308},
  year={2015},
  publisher={IEEE}
}

@ARTICLE{lucente07,
  AUTHOR =       {Gianluca Lucente and Marcello Montanari and Carlo Rossi},
  TITLE =        {Modelling of an automated manual transmission system},
  JOURNAL =      {Mechatronics},
  YEAR =         {2007},
  volume =       {17},
  number =       {73-91},
}

@ARTICLE{lukic04,
  AUTHOR =       {Srdjan M. Lukic and Ali Emadi},
  TITLE =        {Effects of Drivetrain Hybridization on Fuel Economy and Dynamic Performance of Parallel Hybrid Electric Vehicles},
  JOURNAL =      {IEEE Transactions on Vehicular Technology},
  YEAR =         {2004},
  volume =       {53},
  number =       {2},
  pages =        {385-389},
}

% M ------------------------------------------------------------------------------------
@article{maamria19,
  title={Optimal predictive eco-driving cycles for conventional, electric, and hybrid electric cars},
  author={Maamria, Djamaleddine and Gillet, Kristan and Colin, Guillaume and Chamaillard, Yann and Nouillant, C{\'e}dric},
  journal={IEEE Transactions on Vehicular Technology},
  volume={68},
  number={7},
  pages={6320--6330},
  year={2019},
  publisher={IEEE}
}

@ARTICLE{macian18,
  AUTHOR =       {V Macian and C Guardiola and B Pla and A Reig},
  TITLE =        {Application and benchmarking of a direct method to optimize the fuel consumption of a diesel electric locomotive},
  JOURNAL =      {Proc IMechE Part F: J Rail and Rapid Transit},
  YEAR =         {2018},
  volume =       {},
  number =       {},
  pages =        {},
  doi =          {10.1177/0954409718772133},
}

@ARTICLE{mahamud11,
  AUTHOR =       {Rajib Mahamud and Chanwoo Park},
  TITLE =        {Reciprocating air flow for {Li-ion} battery thermal management to improve temperature uniformity},
  JOURNAL =      {Journal of Power Sources},
  YEAR =         {2011},
  volume =       {196},
  number =       {13},
  pages =        {5685-5696},
}

@CONFERENCE{mapelli09,
  AUTHOR =       {Ferdinando Mapelli and Marco Mauri and Davide Tarsitano},
  TITLE =        {Energy control strategies comparison for a city car Plug-In {HEV}},
  booktitle =    {Industrial Electronics, IECON '09. 35th Annual Conference of IEEE.},
  YEAR =         {2009},
}

@ARTICLE{markel02,
  AUTHOR =       {T. Markel and A. Brooker and T. Hendricks and V. Johnson and K. Kelly and B. Kramer and M. O'Keefe and S. Sprik and K. Wipke},
  TITLE =        {{ADVISOR}: a systems analysis tool for advanced vehicle modeling},
  JOURNAL =      {Journal of Power Sources},
  YEAR =         {2002},
  volume =       {110},
  number =       {2},
  pages =        {255-266},
}

@TECHREPORT{martin14,
  author =       {Sebastian Martin and Christian Beidl and Rolf Mueller},
  title =        {Responsiveness of a 30 Bar {BMEP} 3-Cylinder Engine: Opportunities and Limits of Turbocharged Downsizing},
  institution =  {SAE International},
  type =         {Technical Paper},
  year =         {2014},
  number =       {2014-01-1646},
}


@ARTICLE{mayne00,
  AUTHOR =       {D.Q. Mayne and J.B. Rawlings and C.V. Rao and P.O.M. Scokaert},
  TITLE =        {Constrained model predictive control : Stability and optimality},
  JOURNAL =      {Automatica},
  YEAR =         {2000},
  volume =       {36},
  number =       {6},
  pages =        {789-814},
}

@ARTICLE{mcshane39,
  AUTHOR =       {E. J. McShane},
  TITLE =        {On Multipliers for {Lagrange} Problems},
  JOURNAL =      {American Journal of Mathematics},
  YEAR =         {1939},
  volume =       {61},
  number =       {4},
  pages =        {809-819},
}

@ARTICLE{mierlo01,
  AUTHOR =       {J. Van Mierlo and G. Maggetto},
  TITLE =        {Vehicle simulation program: a tool to evaluate hybrid power management strategies based on an innovative iteration algorithm},
  JOURNAL =      {Proc Instn Mech Engrs},
  YEAR =         {2001},
  volume =       {215 Part D},
}

@BOOK{nocedal06,
  AUTHOR =       {J. Nocedal and S. J. Wright},
  TITLE =        {Numerical Optimization},
  PUBLISHER =    {Springer},
  YEAR =         {2006},
  pages =        {0-387},
}


@CONFERENCE{miller05,
  AUTHOR =       {John M. Miller and Patrick J. McCleer and Michael Everett and Elias G. Strangas},
  TITLE =        {Ultracapacitor Plus Battery Energy Storage System Sizing Methodology for {HEV} Power Split Electronic {CVT}'s},
  booktitle =    {IEEE ISIE, Dubrovnik, Croatia},
  YEAR =         {2005},
}

@ARTICLE{miller07,
  AUTHOR =       {John M. Miller},
  TITLE =        {Energy storage technology markets and application's: ultracapacitors in combination with lithium-ion},
  JOURNAL =      {Internatonal Conference on Power Electronics},
  YEAR =         {2007},
  pages =        {16-22},
}

@ARTICLE{minguez13,
  AUTHOR =       {Roberto M�nguez and Antonio J. Conejo and Enrique Castillo},
  TITLE =        {Optimal engineering design via {B}enders' decomposition},
  JOURNAL =      {Annals of Operations Research},
  volume =       {210},
  number =       {1},
  YEAR =         {2013},
  pages =        {273-293},
  publisher =    {Springer US},
  issn =         {0254-5330},
}

@BOOK{montgomery03,
  AUTHOR =       {Douglas C. Montgomery and George C. Runger},
  TITLE =        {Applied Statistics and Probability for Engineers},
  PUBLISHER =    {John Wiley and Sons, Inc., USA},
  YEAR =         {2003},
}

@BOOK{montgomery09,
  AUTHOR =       {Douglas C. Montgomery},
  TITLE =        {Design and Analysis of Experiments},
  PUBLISHER =    {John Wiley \& Sons, Inc.},
  EDITION =      {7},
  YEAR =         {2009},
}

@CONFERENCE{moore97,
  author =       {Timothy C. Moore},
  title =        {{HEV} Control Strategy: Implications of Performance Criteria, System Configuration and Design, and Component Selection},
  booktitle =    {Proceedings of the American Control Conference, Albuquerque, New Mexico},
  year =         {1997},
}

@CONFERENCE{motloch02,
  author =       {Chester G. Motloch and Jon P. Christophersen and Jeffrey R. Belt and Randy B. Wright and Gary L. Hunt and Raymond A. Sutula and Tien Duong and Thomas J. Tartamella and Harold J. Haskins and Ted J. Miller},
  title =        {High-Power Battery Testing Procedures and Analytical Methodologies for {HEV}'s},
  booktitle =    {Future Car Congress, Arlington, Virginia},
  year =         {2002},
}

@ARTICLE{moura10,
  AUTHOR =       {Scott J. Moura and Duncan S. Callaway and Hosam K. Fathy and Jeffrey L. Stein},
  TITLE =        {Tradeoffs between battery energy capacity and stochastic optimal power management in plug-in hybrid electric vehicles},
  JOURNAL =      {Journal of Power Sources},
  YEAR =         {2010},
  volume =       {195},
  number =       {9},
  pages =        {2979-2988},
}

@CONFERENCE{murgovski10a,
  AUTHOR =       {Nikolce Murgovski and Jonas Sj\"oberg and Jonas Fredriksson},
  TITLE =        {A tool for generating optimal control laws for hybrid electric powertrains},
  booktitle =    {IFAC Symposium on Advances in Automotive Control},
  YEAR =         {2010},
  address =      {Munich, Germany},
}

@CONFERENCE{murgovski10b,
  AUTHOR =       {Nikolce Murgovski and Jonas Sj\"oberg and Jonas Fredriksson},
  TITLE =        {Automatic Simplification of Hybrid Powertrain Models for Use in Optimization},
  booktitle =    {International Symposium on Advanced Vehicle Control},
  YEAR =         {2010},
  address =      {Loughborough, UK},
}

@CONFERENCE{murgovski10c,
  AUTHOR =       {Nikolce Murgovski and Jonas Fredriksson and Jonas Sj\"oberg},
  TITLE =        {Hybrid powertrain concept evaluation using optimization},
  booktitle =    {Electric Vehicle Symposium (EVS-25)},
  YEAR =         {2010},
  address =      {Shenzhen, China},
}

@CONFERENCE{murgovski11IFACWC,
  AUTHOR =       {Nikolce Murgovski and Lars Johannesson and Jonas Hellgren and Bo Egardt and Jonas Sj\"oberg},
  TITLE =        {Convex optimization of charging infrastructure design and component sizing of a plug-in series {HEV} powertrain},
  booktitle =    {IFAC World Congress},
  YEAR =         {2011},
  address =      {Milan, Italy},
}

@ARTICLE{murgovski11IJHV,
  AUTHOR =       {Nikolce Murgovski and Jonas Sj\"oberg and Jonas Fredriksson},
  TITLE =        {A methodology and a tool for evaluating hybrid electric powertrain configurations},
  JOURNAL =      {Int. J. Electric and Hybrid Vehicles},
  YEAR =         {2011},
  volume =       {3},
  number =       {3},
  pages =        {219-245},
}

@ARTICLE{murgovski12Mec,
  AUTHOR =       {Nikolce Murgovski and Lars Johannesson and Jonas Sj\"oberg and Bo Egardt},
  TITLE =        {Component sizing of a plug-in hybrid electric powertrain via convex optimization},
  JOURNAL =      {Mechatronics},
  YEAR =         {2012},
  volume =       {22},
  number =       {1},
  pages =        {106-120},
}

@ARTICLE{murgovski16,
  AUTHOR =       {Nikolce Murgovski and Bo Egardt and Magnus Nilsson},
  TITLE =        {Cooperative energy management of automated vehicles},
  JOURNAL =      {Control Engineering Practice},
  YEAR =         {2016},
  volume =       {57},
  pages =        {84-98},
}

@CONFERENCE{murgovski12ECOSM,
  author =       {Nikolce Murgovski and Lars Johannesson and Jonas Sj\"oberg},
  title =        {Convex modeling of energy buffers in power control applications},
  booktitle =    {IFAC Workshop on Engine and Powertrain Control, Simulation and Modeling (E-CoSM)},
  year =         {2012},
  address =      {Rueil-Malmaison, Paris, France},
}

@CONFERENCE{murgovski12CDC,
  author =       {Nikolce Murgovski and Lars Johannesson and Anders Grauers and Jonas Sj\"oberg},
  title =        {Dimensioning and control of a thermally constrained double buffer plug-in {HEV} powertrain},
  booktitle =    {IEEE Conference on Decision and Control},
  year =         {2012},
  address =      {Maui, Hawaii},
}

@PHDTHESIS{murgovski12PhD,
  author =       {Nikolce Murgovski},
  title =        {Optimal Powertrain Dimensioning and Potential Assessment of Hybrid Electric Vehicles},
  school =       {Chalmers University of Technology},
  year =         {2012},
  address =      {Gothenburg, Sweden},
}

@ARTICLE{murgovski13TVT,
  author =       {Nikolce Murgovski and Lars Johannesson and Jonas Sj\"oberg},
  title =        {Engine on/off control for dimensioning hybrid electric powertrains via convex optimization},
  journal =      {IEEE Transactions on Vehicular Technology},
  year =         {2013},
  volume =       {62},
  number =       {7},
  pages =        {2949-2962},
}

@CONFERENCE{murgovski13china,
  author =       {Nikolce Murgovski and Xiaosong Hu and Lars Johannesson and Bo Egardt},
  title =        {Filtering driving cycles for assessment of electrified vehicles},
  booktitle =    {Workshop for new energy vehicle dynamic system and control technology},
  year =         {2013},
  address =      {Beijing, China},
}

@ARTICLE{murgovski14TVT,
  author =       {Nikolce Murgovski and Lars Johannesson and Bo Egardt},
  title =        {Optimal battery dimensioning and control of a {CVT} {PHEV} powertrain},
  journal =      {IEEE Transactions on Vehicular Technology},
  year =         {2014},
  volume =       {63},
  number =       {5},
  pages =        {2151-2161},
}

@CONFERENCE{murgovski14IFACWC,
  author =       {Nikolce Murgovski and Xiaosong Hu and Bo Egardt},
  title =        {Computationally efficient energy management of a planetary gear hybrid electric vehicle},
  booktitle =    {IFAC World Congress},
  year =         {2014},
  address =      {Cape Town, South Africa},
}

@ARTICLE{murgovski14TCST,
  author =       {Nikolce Murgovski and Markus Grahn and Lars Johannesson and Tomas McKelvey},
  title =        {Automated engine calibration of hybrid electric vehicles},
  journal =      {IEEE Transactions on Control Systems Technology},
  year =         {2014},
  doi =          {10.1109/TCST.2014.2360920},
}

@INBOOK{murgovski15bookch,
  author =       {Nikolce Murgovski and Xiaosong Hu and Lars Johannesson and Bo Egardt},
  title =        {Combined design and control optimization of hybrid vehicles},
  booktitle =    {Handbook of Clean Energy Systems},
  publisher =    {John Wiley & Sons, Ltd},
  year =         {2015},
  doi =          {10.1002/9781118991978.hces110},
  isbn =         {9781118991978},
}

@CONFERENCE{murgovski15ACC,
  author =       {Nikolce Murgovski and Lars Johannesson and Xiaosong Hu and Bo Egardt and Jonas Sj\"oberg},
  title =        {Convex relaxations in the optimal control of electrified vehicles},
  booktitle =    {American Control Conference},
  year =         {2015},
  address =      {Chicago, USA},
}

@CONFERENCE{murgovski15CDCa,
  author =       {Nikolce Murgovski and Jonas Sj\"oberg},
  title =        {Predictive cruise control with autonomous overtaking},
  booktitle =    {Conference on Decision and Control},
  year =         {2015},
  address =      {Osaka, Japan},
}

@CONFERENCE{murgovski15CDCb,
  author =       {Nikolce Murgovski and Gabriel Rodrigues de Campos and Jonas Sj\"oberg},
  title =        {Convex modeling of conflict resolution at traffic intersections},
  booktitle =    {Conference on Decision and Control},
  year =         {2015},
  address =      {Osaka, Japan},
}

@CONFERENCE{musardo05,
  AUTHOR =       {Cristian Musardo and Giorgio Rizzoni and Benedetto Staccia},
  TITLE =        {{A-ECMS}: An Adaptive Algorithm for Hybrid Electric Vehicle Energy Management},
  BOOKTITLE =    {IEEE Conference on Decision and Control, and the European Control Conference},
  YEAR =         {2005},
  address =      {Seville, Spain},
}

% N ------------------------------------------------------------------------------------

@BOOK{naidu02,
  AUTHOR =       {Desineni Subbaram Naidu},
  TITLE =        {Optimal Control Systems},
  PUBLISHER =    {CRC Press},
  YEAR =         {2002},
}

@TECHREPORT{nakayama03,
  author =       {S. Nakayama and T. Fukuma and A. Matsunaga and T. Miyake and T. Wakimoto},
  title =        {A New Dynamic Combustion Control Method Based on Charge Oxygen Concentration for {D}iesel Engines},
  institution =  {SAE International},
  type =         {Technical Paper},
  year =         {2003},
  number =       {2003-01-3181},
}

@ARTICLE{nakayama08,
  AUTHOR =       {S. Nakayama and T. Ibuki and H. Hosaki and H. Tominaga},
  TITLE =        {An Application of Model Based Combustion Control to Transient Cycle-by-Cycle {D}iesel Combustion},
  JOURNAL =      {SAE Int. J. Engines},
  YEAR =         {2008},
  volume =       {1},
  number =       {1},
  pages =        {850-860},
}

@ARTICLE{narasimhan86,
  AUTHOR =       {S. Narasimhan and R. S. H. Mah and A. C. Tamhane and J. W. Woodward and J. C. Hale},
  TITLE =        {A composite statistical test for detecting changes of steady states},
  JOURNAL =      {AIChE Journal},
  YEAR =         {1986},
  volume =       {32},
  number =       {9},
  pages =        {1409-1418},
}

@ARTICLE{narasimhan87,
  AUTHOR =       {S. Narasimhan and Chen Shan Kao and R. S. H. Mah},
  TITLE =        {Detecting Changes of Steady States Using the Mathematical Theory of Evidence},
  JOURNAL =      {AIChE Journal},
  YEAR =         {1987},
  volume =       {33},
  number =       {11},
}

@CONFERENCE{neuman08,
  AUTHOR =       {Magnus Neuman and Henrik Sandberg and Bo Wahlberg and Anders Folkesson},
  TITLE =        {Modelling and Control of Series {HEV}s Including Resistive Losses and Varying Engine Efficiency},
  booktitle =    {SAE International},
  YEAR =         {2008},
}

@ARTICLE{ngo12,
  AUTHOR =       {Viet Ngo and Theo Hofman and Maarten Steinbuch and Alex Serrarens},
  TITLE =        {Optimal Control of the Gearshift Command for Hybrid Electric Vehicles},
  JOURNAL =      {IEEE Transactions On Vehicular Technology},
  YEAR =         {2012},
  volume =       {61},
  number =       {8},
  pages =        {3531-3543},
}

@CONFERENCE{nilsson13,
  author =       {Julia Nilsson and Mohammad Ali and Paolo Falcone and Jonas Sj\"oberg},
  title =        {Predictive manoeuvre generation for automated driving},
  booktitle =    {Intelligent Transportation Systems (ITSC)},
  year =         {2013},
  address =      {The Hague, The Netherlands},
}

@CONFERENCE{nilsson14,
  author =       {Julia Nilsson and Yiqi Gao and Ashwin Carvalho and Francesco Borrelli},
  title =        {Manoeuvre generation and control for automated highway driving},
  booktitle =    {IFAC World Congress},
  year =         {2014},
  address =      {Cape Town, South Africa},
}

@CONFERENCE{nilsson15,
  author =       {Magnus Nilsson and Nikolce Murgovski and Lars Johannesson},
  title =        {Combined platooning and energy management with high integrity},
  booktitle =    {International Conference on Energy Efficient Vehicles (ECEEV)},
  year =         {2015},
  address =      {Dresden, Germany},
}

@CONFERENCE{norlund02,
  author =       {Erik Nordlund and Chandur Sadarangani},
  title =        {The Four-Quadrant Energy Transducer},
  booktitle =    {Industry Applications Conference},
  year =         {2002},
  address =      {Pittsburgh, PA, USA},
}

@BOOK{nowak05,
  AUTHOR =       {Ivo Nowak},
  TITLE =        {Relaxation and Decomposition Methods for Mixed Integer Nonlinear Programming},
  PUBLISHER =    {Birkh\"auser Basel},
  YEAR =         {2005},
}

@ARTICLE{nuesch14,
  author =       {Tobias N\"uesch and Philipp Elbert and Michael Flankl and Christopher Onder and Lino Guzzella},
  title =        {Convex Optimization for the Energy Management of Hybrid Electric Vehicles Considering Engine Start and Gearshift Costs},
  journal =      {Energies},
  year =         {2014},
  volume =       {7},
  number =       {2},
  pages =        {834-856},
}

@BOOK{nunney07,
  AUTHOR =       {M. J. Nunney},
  TITLE =        {Light and Heavy Vehicle Technology},
  PUBLISHER =    {Butterworth-Heinemann},
  YEAR =         {2007},
}

% O ------------------------------------------------------------------------------------

@ARTICLE{oecd13,
  author =       {{OECD/ITF}},
  title =        {{ITF} Transport Outlook 2013},
  year =         {2013},
}

@book{international2008co2,
  title={CO2 Emissions from Fuel Combustion: 1972},
  author={International Energy Agency Staff},
  year={2008},
  publisher={Organization for Economic}
}

@ARTICLE{oecdiea18,
   author = "International Energy Agency",
   title = "CO2 Emissions from Fuel Combustion 2018",
   year = "2018",
   pages = 515, 
}

@BOOK{oecditf19,
  author = "International Transport Forum",
  title = "ITF Transport Outlook 2019",
  year = "2019",
  pages = 200,
  doi =          {10.1787/9789282103937-en},
  ISBN =         {9789282103937},
  publisher =    {OECD Publishing/ITF, Paris, France, Tech, Rep.},
}

@article{ohtsuka04,
  title={A continuation/{GMRES} method for fast computation of nonlinear receding horizon control},
  author={Ohtsuka, Toshiyuki},
  journal={Automatica},
  volume={40},
  number={4},
  pages={563--574},
  year={2004},
  publisher={Elsevier}
}


@ARTICLE{opila12,
  author =       {Daniel F. Opila and Xiaoyong Wang and Ryan McGee and R. Brent Gillespie and Jeffrey A. Cook and Jessy W. Grizzle},
  title =        {An Energy Management Controller to Optimally Trade Off Fuel Economy and Drivability for Hybrid Vehicles},
  journal =      {IEEE Transactions on Control Systems Technology},
  year =         {2012},
  volume =       {20},
  number =       {6},
  pages =        {1490-1505},
}

@MISC{orion,
  author =       {{Daimler Buses North America}},
  title =        {{Orion VII Hybrid}},
  howpublished = {\url{http://www.orionbus.com}},
  note =         {Accessed March 2012},
}

@ARTICLE{ott12,
  author =       {Tobias Ott and Florian Zurbriggen and Christopher Onder and Lino Guzzella},
  title =        {Cycle-averaged efficiency of hybrid electric vehicles},
  journal =      {Proc IMechE Part D: Journal of Automobile Engineering},
  year =         {2012},
  doi =          {10.1177/0954407012447508},
  pages =        {1-9},
}

% P ------------------------------------------------------------------------------------

@BOOK{pacejka02,
  AUTHOR =       {Hans B Pacejka},
  TITLE =        {Tyre and Vehicle Dynamics},
  PUBLISHER =    {Buttherworth-Heinemann},
  YEAR =         {2002},
}

@CONFERENCE{pachernegg69,
  author =       {S. J. Pachernegg},
  title =        {A closer look at the Willans-line},
  year =         {1969},
  publisher =    {SAE Technical Paper},
  note =         {doi:10.4271/690182},
}

@article{padilla18,
  title={A global optimal solution to the eco-driving problem},
  author={Padilla, GP and Weiland, Siep and Donkers, MCF},
  journal={IEEE control systems letters},
  volume={2},
  number={4},
  pages={599--604},
  year={2018},
  publisher={IEEE}
}

@CONFERENCE{paganelli01,
  AUTHOR =       {G. Paganelli and S. Delprat and T. M. Guerra and J. Rimaux and J.J. Santin},
  TITLE =        {Control development for a hybrid-electric sport-utility vehicle: strategy, implementation and field test results},
  booktitle =    {Proceedings of the American Control Conference},
  YEAR =         {2001},
}

@INPROCEEDINGS{paganelli02,
  AUTHOR =       {G. Paganelli and S. Delprat and T. M. Guerra and J. Rimaux and J.J. Santin},
  TITLE =        {Equivalent Consumption Minimization Strategy for Parallel Hybrid Powertrains},
  booktitle =    {IEEE Vehicular Technology Conference},
  YEAR =         {2002},
  pages =        {2076-2081},
}

@CONFERENCE{park03,
  author =       {Chanwoo Park and Arun K. Jaura},
  title =        {Dynamic Thermal Model of {Li-ion} Battery for Predictive Behavior in Hybrid and Fuel Cell Vehicles},
  booktitle =    {Future Transportation Technology Conference, Costa Mesa, California},
  year =         {2003},
}

@CONFERENCE{parsons01,
  author =       {Ken Parsons},
  title =        {The estimation of metabolic heat for use in the assessment of thermal comfort},
  booktitle =    {Moving Thermal Comfort Standards into the 21st Century, Windsor},
  year =         {2001},
  address =      {UK},
}

@CONFERENCE{passenberg09,
  author =       {Benjamin Passenberg and Peter Kock and Olaf Stursberg},
  title =        {Combined time and fuel optimal driving of trucks based on a hybrid model},
  booktitle =    {European Control Conference},
  year =         {2009},
  pages  =       {4955-4960},
  address =      {Budapest, Hungary},
}

@ARTICLE{peppard74,
  author =       {Lloyd E. Peppard},
  title =        {String stability of relative-motion {PID} vehicle control systems},
  journal =      {IEEE Transactions on Automatic Control},
  year =         {1974},
  volume =       {19},
  number =       {5},
  pages =        {579-581},
}

@ARTICLE{pesaran02,
  AUTHOR =       {A. Pesaran},
  TITLE =        {Battery thermal models for hybrid vehicle simulations},
  JOURNAL =      {Journal of Power Sources},
  YEAR =         {2002},
  volume =       {110},
  number =       {2},
  pages =        {377-382},
}

@ARTICLE{peters13,
  author =       {Diane L. Peters and Panos Y. Papalambros and A. Galip Ulsoy},
  title =        {Sequential co-design of an artifact and its controller via control proxy functions},
  journal =      {Mechatronics},
  year =         {2013},
  volume =       {23},
  number =       {4},
  pages =        {409-418},
}

@ARTICLE{peterson10,
  AUTHOR =       {Scott B. Peterson and Jay Apt and J.F. Whitacre},
  TITLE =        {Lithium-ion battery cell degradation resulting from realistic vehicle and vehicle-to-grid utilization},
  JOURNAL =      {Journal of Power Sources},
  YEAR =         {2010},
  volume =       {195},
  number =       {8},
  pages =        {2385-2392},
}

@CONFERENCE{pisu05,
  AUTHOR =       {Pierluigi Pisu and Giorgio Rizzoni},
  TITLE =        {A Supervisory Control Strategy for Series Hybrid Electric Vehicles with Two Energy Storage Systems},
  booktitle =    {IEEE Vehicle Power and Propulsion Conference},
  YEAR =         {2005},
}

@ARTICLE{pisu07,
  AUTHOR =       {Pierluigi Pisu and Giorgio Rizzoni},
  TITLE =        {A Comparative Study Of Supervisory Control Strategies for Hybrid Electric Vehicles},
  JOURNAL =      {IEEE Transactions on Control Systems Technology},
  YEAR =         {2007},
  volume =       {15},
  number =       {3},
  pages =        {506-518},
}

@ARTICLE{pohl07,
  AUTHOR =       {J. Pohl and W. Birk and L. Westervall},
  TITLE =        {A driver-distraction-based lane-keeping assistance system},
  JOURNAL =      {J. Systems and Control Engineering},
  YEAR =         {2007},
  volume =       {221},
  pages =        {541-552},
}

@BOOK{pontryagin62,
  AUTHOR =       {L. S. Pontryagin and V. G. Boltyanskii and R. V. Gamkrelidze and E. F. Mishchenko},
  TITLE =        {The Mathematical Theory of Optimal Processes},
  PUBLISHER =    {Interscience Publishers},
  YEAR =         {1962},
}

@ARTICLE{pourabdollah13,
  AUTHOR =       {Mitra Pourabdollah and Nikolce Murgovski and Anders Grauers and Bo Egardt},
  TITLE =        {Optimal sizing of a parallel {PHEV} powertrain},
  JOURNAL =      {IEEE Transactions on Vehicular Technology},
  YEAR =         {2013},
  volume =       {62},
  number =       {6},
  pages =        {2469-2480},
}

@CONFERENCE{pourabdollah14,
  author =       {Mitra Pourabdollah and Nikolce Murgovski and Anders Grauers and Bo Egardt},
  title =        {An Iterative Dynamic Programming/convex Optimization Procedure for Optimal Sizing and Energy Management of {PHEVs}},
  booktitle =    {IFAC World Congress},
  year =         {2014},
  pages  =       {6606-6611},
  address =      {Cape Town, South Africa},
}

% Q ------------------------------------------------------------------------------------

@ARTICLE{qi07,
  AUTHOR =       {Zhao-gang Qi and Jiang-ping Chen and Zhi-jiu Chen},
  TITLE =        {Analysis and simulation of mobile air conditioning system coupled with engine cooling system},
  JOURNAL =      {Energy Conversion and Management},
  YEAR =         {2007},
  volume =       {48},
  number =       {4},
  pages =        {1176-1184},
}

% R ------------------------------------------------------------------------------------

@TECHREPORT{rao79,
  AUTHOR =       {Harish S. Rao and A. I. Cohen and J. A. Tennant and K. L. Van Voorhies},
  TITLE =        {Engine Control Optimization Via Nonlinear Programming},
  institution =  {SAE International},
  type =         {Technical Paper},
  YEAR =         {1979},
  number =       {790177},
}

@ARTICLE{reyer02,
  author =       {Julie A. Reyer and Panos Y. Papalambros},
  title =        {Combined Optimal Design and Control With Application to an Electric {DC} Motor},
  journal =      {Journal of Mechanical Design},
  year =         {2002},
  volume =       {142},
  number =       {2},
  pages =        {183-191},
}

@CONFERENCE{rhinehart95,
  AUTHOR =       {R. Russell Rhinehart},
  TITLE =        {A novel method for automated identification of steady state},
  BOOKTITLE =    {Proceedings of the American Control Conference},
  YEAR =         {1995},
  address =      {Seattle, Washington},
}

@TECHREPORT{rishavy77,
  AUTHOR =       {E. Rishavy and S. Hamilton and J. Ayers and M. Keane},
  TITLE =        {Engine Control Optimization for Best Fuel Economy with emission Constraints},
  institution =  {SAE International},
  type =         {Technical Paper},
  YEAR =         {1977},
  number =       {770075},
}

@ARTICLE{rizzoni99,
  AUTHOR =       {Giorgio Rizzoni and Lino Guzzella and Bernd M. Baumann},
  TITLE =        {Unified Modeling of Hybrid Electric Vehicle Drivetrains},
  JOURNAL =      {IEEE/ASME Trans. Mechatron.},
  YEAR =         {1999},
  volume =       {4},
  number =       {3},
  pages =        {246-257},
}

@CONFERENCE{rotenberg08,
  AUTHOR =       {Dean Rotenberg and Ardalan Vahidi and Ilya Kolmanovsky},
  TITLE =        {Ultracapacitor Assisted Powertrains: Modeling, Control, Sizing, and The Impact on Fuel Economy},
  booktitle =    {American Control Conference, Seattle, Washington, USA},
  YEAR =         {2008},
}

@ARTICLE{rutquist08,
  author =       {Per Rutquist and Claes Breitholtz and Torsten Wik},
  title =        {On the infinite time solution to state-constrained stochastic optimal control problems},
  journal =      {Automatica},
  year =         {2008},
  volume =       {44},
  number =       {7},
  pages =        {1800-1805},
}

% S ------------------------------------------------------------------------------------

@ARTICLE{sager09,
  AUTHOR =       {Sebastian Sager},
  TITLE =        {Reformulations and algorithms for the optimization of switching decisions in nonlinear optimal control},
  JOURNAL =      {Journal of Process Control},
  YEAR =         {2009},
  volume =       {19},
  number =       {8},
  pages =        {1238-1247},
}

@CONFERENCE{sargent96,
  AUTHOR =       {Robert G. Sargent},
  TITLE =        {Verifying and Validating Simulation Models},
  BOOKTITLE =    {Proceedings of the conference on Winter simulation},
  YEAR =         {1996},
  pages  =       {55-64},
  address =      {Coronado, California},
}

@CONFERENCE{sargent96b,
  AUTHOR =       {Robert G. Sargent},
  TITLE =        {Some subjective validation methods using graphical displays of data},
  BOOKTITLE =    {Proceedings of the conference on Winter simulation},
  YEAR =         {1996},
  pages  =       {345-351},
  address =      {Coronado, California},
}

@ARTICLE{sauer08,
  AUTHOR =       {Dirk Uwe Sauer and Heinz Wenzl},
  TITLE =        {Comparison of different approaches for lifetime prediction of electrochemical systems---{U}sing lead-acid batteries as example},
  JOURNAL =      {Journal of Power Sources},
  YEAR =         {2008},
  volume =       {176},
  number =       {2},
  pages =        {534-546},
}

@article{sharma20,
  title={Optimal eco-driving of a heavy-duty vehicle behind a leading heavy-duty vehicle},
  author={Sharma, Nalin Kumar and Hamednia, Ahad and Murgovski, Nikolce and Gelso, Esteban R and Sj{\"o}berg, Jonas},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  volume={22},
  number={12},
  pages={7792--7803},
  year={2020},
  publisher={IEEE}
}

@TECHREPORT{schijndel11,
  author =       {Margriet van Schijndel-de Nooij and Bastiaan Krosse and Thijs van den Broek and Sander Maas and Ellen van Nunen and Han Zwijnenberg and Anna Schieben and Henning Mosebach and Nick Ford and Mike McDonald and David Jeffery and Jinan Piao and Javier Sanchez},
  title =        {Definition of necessary vehicle and infrastructure systems for automated driving},
  institution =  {European Commission},
  year =         {2011},
  number =       {2010/0064},
}

@article{schittkowski83,
  title={On the convergence of a sequential quadratic programming method with an augmented Lagrangian line search function},
  author={Schittkowski, Klaus},
  journal={Mathematische Operationsforschung und Statistik. Series Optimization},
  volume={14},
  number={2},
  pages={197--216},
  year={1983},
  publisher={Taylor \& Francis}
}


@MISC{schmidt96,
  author =       {Michael R. Schmidt},
  title =        {Two-mode, split power, electro-mechanical transmission},
  year =         {1996},
}

@TECHREPORT{schmitz94,
  AUTHOR =       {G. Schmitz and U. Oligschl\"{a}ger and G. Eifles},
  TITLE =        {Automated System for Optimized Calibration of Engine Management Systems},
  institution =  {SAE International},
  type =         {Technical Paper},
  YEAR =         {1994},
  number =       {940151},
}

@PHDTHESIS{schofield08,
  AUTHOR =       {Brad Schofield},
  TITLE =        {ModelBased Vehicle Dynamics Control for Active Safety},
  SCHOOL =       {Department of Automatic Control Lund University},
  YEAR =         {2008},
  address =      {Lund},
}

@ARTICLE{schouten03,
  AUTHOR =       {Niels J Schouten and Mutasim A Salman and Naim A Kheir},
  TITLE =        {Energy management strategies for parallel hybrid vehicles using fuzzy logic},
  JOURNAL =      {Control Engineering Practice},
  YEAR =         {2003},
  volume =       {11},
  number =       {2},
  pages =        {171-177},
}

@CONFERENCE{schreiber07,
  AUTHOR =       {A. Schreiber and R. Isermann},
  TITLE =        {Identification methods for experimental nonlinear modeling of combustion engines},
  booktitle =    {IFAC Symposium on Advances in Automotive Control},
  YEAR =         {2007},
}

@ARTICLE{schwarzkopf77,
  AUTHOR =       {A.B. Schwarzkopf and R.B. Leipnik},
  TITLE =        {Control of highway vehicles for minimum fuel consumption over varying terrain},
  JOURNAL =      {Transportation Research},
  YEAR =         {1977},
  volume =       {11},
  number =       {4},
  pages =        {279-286},
}

@CONFERENCE{sciarretta04a,
  author =       {A. Sciarretta and L. Guzzella and M. Back},
  title =        {A real-time optimal control strategy for parallel hybrid vehicles with on-board estimation of control parameters},
  booktitle =    {Proc. IFAC Symp. Advances Automotive Control},
  year =         {2004},
  address =      {Salerno, Italy},
}

@ARTICLE{sciarretta04,
  AUTHOR =       {Antonio Sciarretta and Michael Back and Lino Guzzella},
  TITLE =        {Optimal Control of Parallel Hybrid Electric Vehicles},
  JOURNAL =      {IEEE Transactions on Control Systems Technology},
  YEAR =         {2004},
  volume =       {12},
  number =       {3},
  pages =        {352-363},
}

@ARTICLE{sciarretta07,
  AUTHOR =       {Antonio Sciarretta and Lino Guzzella},
  TITLE =        {Control of Hybrid Electric Vehicles},
  JOURNAL =      {IEEE Control Systems Magazine},
  YEAR =         {2007},
  volume =       {27},
  number =       {2},
  pages =        {60-70},
}

@ARTICLE{sciarretta15,
  AUTHOR =       {Antonio Sciarretta and Giovanni De Nunzio and Luis Leon Ojeda},
  TITLE =        {Optimal Ecodriving Control: Energy-Efficient Driving of Road Vehicles as an Optimal Control Problem},
  JOURNAL =      {IEEE Control Systems Magazine},
  YEAR =         {2015},
  volume =       {35},
  number =       {5},
  pages =        {71-90},
}

@MISC{sdpt3_06,
  AUTHOR =       {K. C. Toh and R. H. T\"ut\"unc\"u and M. J. Todd},
  TITLE =        {On the implementation and usage of {SDPT3} - a {Matlab} software package for semidefinite-quadratic-linear programming, version 4.0},
  YEAR =         {2006},
}

@ARTICLE{sedumi02,
  AUTHOR =       {Yam Labit and Dimitri Peaucelle and Didier Henrion},
  TITLE =        {{SeDuMi} Interface 1.02: a tool for solving {LMI} problems with {SeDuMi}},
  JOURNAL =      {IEEE International Symposium on Computer Aided Control System Design Proceedings},
  YEAR =         {2002},
  pages =        {272-277},
}

@CONFERENCE{serrao05,
  AUTHOR =       {Lorenzo Serrao and Zakaria Chehab and Yann Guezennec and Giorgio Rizzoni},
  TITLE =        {An aging model of {Ni-MH} batteries for hybrid electric vehicles},
  booktitle =    {IEEE Vehicle Power and Propulsion Conference},
  YEAR =         {2005},
}

@CONFERENCE{serrao11,
  author =       {Lorenzo Serrao and Simona Onori and Antonio Sciarretta and Yann Guezennec and Giorgio Rizzoni},
  title =        {Optimal energy management of hybrid electric vehicles including battery aging},
  booktitle =    {American Control Conference},
  year =         {2011},
  address =      {San Francisco, USA},
}

@inproceedings{shahed09,
  author =       {S. Shahed and K. Bauer},
  booktitle =    {SAE World Congress \& Exhibition},
  number =       {1},
  pages =        {1347-1358},
  publisher =    {SAE International},
  title =        {Parametric Studies of the Impact of Turbocharging on Gasoline Engine Downsizing},
  volume =       {2},
  year =         {2009},
}

@BOOK{shafer76,
  AUTHOR =       {Glenn Shafer},
  TITLE =        {A Mathematical Theory of Evidence},
  PUBLISHER =    {Princeton University Press},
  YEAR =         {1976},
}

@article{shen20,
  title={A minimum principle-based algorithm for energy-efficient eco-driving of electric vehicles in various traffic and road conditions},
  author={Shen, Daliang and Karbowski, Dominik and Rousseau, Aymeric},
  journal={IEEE Transactions on Intelligent Vehicles},
  volume={5},
  number={4},
  pages={725--737},
  year={2020},
  publisher={IEEE}
}

@BOOK{si04,
  AUTHOR =       {Jennie Si and Andy Barto and Warren Powell and Donald Wunsch},
  TITLE =        {Handbook of Learning and Approximate {Dynamic} {Programming}},
  PUBLISHER =    {IEEE Press, John Wiley \& sons, Inc.},
  YEAR =         {2004},
}

@ARTICLE{silvas17,
  AUTHOR =       {Emilia Silvas and Theo Hofman and Nikolce Murgovski and Pascal Etman and Maarten Steinbuch},
  TITLE =        {Review of optimization strategies for system-level design in hybrid electric vehicles},
  JOURNAL =      {IEEE Transactions on Vehicular Technology},
  YEAR =         {2017},
  volume =       {66},
  number =       {1},
  pages =        {57-70},
}

@ARTICLE{smith06,
  AUTHOR =       {Kandler Smith and Chao-Yang Wang},
  TITLE =        {Power and thermal characterization of a lithium-ion battery pack for hybrid-electric vehicles},
  JOURNAL =      {Journal of Power Sources},
  YEAR =         {2006},
  volume =       {160},
  number =       {1},
  pages =        {662-673},
}

@article{sonoc15,
  title={Opportunities to improve recycling of automotive lithium ion batteries},
  author={Sonoc, Alexandru and Jeswiet, Jack and Soo, Vi Kie},
  journal={Procedia cIRP},
  volume={29},
  pages={752--757},
  year={2015},
  publisher={Elsevier}
}

@CONFERENCE{sundstrom08,
  AUTHOR =       {Olle Sundstr\"om and Lino Guzzella and Patrik Soltic},
  TITLE =        {Optimal Hybridization in Two Parallel Hybrid Electric Vehicles using {Dynamic} {Programming}},
  BOOKTITLE =    {Proceedings of the World Congress The International Federation of Automatic Control},
  YEAR =         {2008},
  address =      {Seoul, Korea},
}

@CONFERENCE{sundstrom09,
  AUTHOR =       {Olle Sundstr\"om and Lino Guzzella},
  TITLE =        {A Generic {Dynamic} {Programming} {Matlab} Function},
  BOOKTITLE =    {18th IEEE International Conference on Control Applications},
  YEAR =         {2009},
  address =      {Saint Petersburg, Russia},
}

@ARTICLE{sundstrom09a,
  AUTHOR =       {Olle Sundstr\"om and Daniel Amb\"uhl and Lino Guzzella},
  TITLE =        {On Implementation of {Dynamic} {Programming} for Optimal Control Problems with Final State Constraints},
  JOURNAL =      {Oil Gas Sci. Technol.},
  YEAR =         {2009},
  volume =       {65},
  number =       {1},
  pages =        {91-102},
}

@PHDTHESIS{sundstrom09thesis,
  AUTHOR =       {Olle Sundstr\"om},
  TITLE =        {Optimal control and design of hybrid-electric vehicles},
  SCHOOL =       {Institute for Dynamic Systems and Control, ETH Zurich},
  YEAR =         {2009},
}

@ARTICLE{sundstrom10,
  AUTHOR =       {Olle Sundstr\"om and Lino Guzzella and Patrik Soltic},
  TITLE =        {Torque-Assist Hybrid Electric Powertrain Sizing: From Optimal Control Towards a Sizing Law},
  JOURNAL =      {IEEE Transactions on Control Systems Technology},
  YEAR =         {2010},
  volume =       {18},
  number =       {4},
  pages =        {837-849},
}

@ARTICLE{solanomartinez12,
  AUTHOR =       {Javier Solano Mart�nez and Robert I. John and Daniel Hissel and Marie-C\'ecile P\'era},
  TITLE =        {A survey-based type-2 fuzzy logic system for energy management in hybrid electrical vehicles},
  JOURNAL =      {Information Sciences},
  YEAR =         {2012},
  volume =       {190},
  number =       {0},
  pages =        {192-207},
}

@ARTICLE{sorrentino11,
  AUTHOR =       {Marco Sorrentino and Gianfranco Rizzo and Ivan Arsie},
  TITLE =        {Analysis of a rule-based control strategy for on-board energy management of series hybrid vehicles},
  JOURNAL =      {Control Engineering Practice},
  YEAR =         {2011},
  volume =       {19},
  number =       {12},
  pages =        {1433-1441},
}

@ARTICLE{sowash09,
  AUTHOR =       {Jennifer Sowash},
  TITLE =        {A Heroic Capacity},
  JOURNAL =      {American Ceramic Society Bulletin},
  YEAR =         {2009},
  volume =       {88},
  number =       {4},
  pages =        {19-25},
}

@TECHREPORT{spendelow12,
  author =       {Jacob Spendelow and Jason Marcinkoski},
  title =        {Fuel Cell System Cost-2012. {DOE} Fuel Cell Technologies Program Record},
  institution =  {US Department of Energy},
  year =         {2012},
  number =       {12020},
}

@article{stroe17,
  title={A two-layer predictive control for hybrid electric vehicles energy management},
  author={Stroe, Nicoleta and Olaru, Sorin and Colin, Guilaume and Ben-Cherif, Karim and Chamaillard, Yann},
  journal={IFAC-PapersOnLine},
  volume={50},
  number={1},
  pages={10058--10064},
  year={2017},
  publisher={Elsevier}
}

@ARTICLE{sturm99,
  AUTHOR =       {Jos F. Sturm},
  TITLE =        {Using {SeDuMi} 1.02, A {Matlab} toolbox for optimization over symmetric cones},
  JOURNAL =      {Optimization Methods and Software},
  YEAR =         {1999},
  volume =       {11},
  number =       {1-4},
  pages =        {635-653},
}

@ARTICLE{svendenius06,
  AUTHOR =       {Jacob Svendenius and Magnus G\"afvert},
  TITLE =        {A Semi-Empirical Dynamic Tire Model for Combined-Slip Forces},
  JOURNAL =      {Vehicle System Dynamics},
  YEAR =         {2006},
  pages = 	     {189-208},
  note =         {Special Issue:AVEC '04: 7th International Symposium on Advanced VEhicle Control 23-27 August 2004 HAN University, Arnhem, The Netherlands},
}

@PHDTHESIS{svendenius07,
  AUTHOR =       {Jacob Svendenius},
  TITLE =        {Tire modeling and Friction Estimation},
  SCHOOL =       {Department of Automatic Control, Lund University},
  address =      {Sweden},
  YEAR =         {2007},
}

@ARTICLE{swaroop96,
  author =       {D. Swaroop and J. K. Hedrick},
  title =        {String Stability of Interconnected Systems},
  journal =      {IEEE Transactions on Automatic Control},
  year =         {1996},
  volume =       {41},
  number =       {3},
  pages =        {349-357},
}

% T ------------------------------------------------------------------------------------

@article{tara10,
  author = {Ehsan Tara and Soheil Shahidinejad and Shaahin Filizadeh and Eric Bibeau},
  journal = {IEEE Transactions on Vehicular Technology},
  number = {6},
  pages = {2786-2794},
  title = {Battery Storage Sizing in a Retrofitted Plug-in Hybrid Electric Vehicle},
  volume = {59},
  year = {2010}
}

@CONFERENCE{tate00,
  AUTHOR =       {Edward D. Tate and Stephen P. Boyd},
  TITLE =        {Finding Ultimate Limits of Performance for Hybrid Electric Vehicles},
  booktitle =    {SAE Technical Paper 2000-01-3099},
  YEAR =         {2000},
}

@article{taylor07,
  author = {Ben Taylor and David Howe},
  journal = {IEEE Transactions on Vehicular Technology},
  number = {6},
  pages = {3674--3681},
  title = {Experimental Characterization of a Supercapacitor-Based Electrical Torque-Boost System for Downsized {ICE} Vehicles},
  volume = {56},
  year = {2007}
}

@ARTICLE{tazelaar12,
  author =       {Edwin Tazelaar and Bram Veenhuizen and Paul van den Bosch and Mark Grimminck},
  title =        {Analytical Solution of the Energy Management for Fuel Cell Hybrid Propulsion Systems},
  journal =      {IEEE Transactions on Vehicular Technology},
  year =         {2012},
  volume =       {61},
  number =       {5},
  pages =        {1986-1998},
}

@ARTICLE{tazelaar12b,
  author =       {E. Tazelaar and Y. Shen and P.A. Veenhuizen and T. Hofman and P.P.J. van den Bosch},
  title =        {Sizing Stack and Battery of a Fuel Cell Hybrid Distribution Truck},
  journal =      {Oil \& Gas Science and Technology - Rev. IFP Energies nouvelles},
  year =         {2012},
  volume =       {67},
  number =       {4},
  pages =        {563-573},
}

@inproceedings{terwen04,
  address =      {Salerno, Italy},
  author =       {S.~Terwen and M.~Back and V.~Krebs},
  booktitle =    {Proc. IFAC Symposium on Advances in Automotive Control},
  title =        {{Predictive powertrain control for heavy duty trucks}},
  year =         {2004},
  pages =        {105-110},
}

@Inbook{themann15,
author="Themann, Philipp
and Zlocki, Adrian
and Eckstein, Lutz",
editor="Siebenpfeiffer, Wolfgang",
title="Energieeffiziente Fahrzeugl{\"a}ngsf{\"u}hrung durch V2X-Kommunikation",
bookTitle="Fahrerassistenzsysteme und Effiziente Antriebe",
year="2015",
publisher="Springer Fachmedien Wiesbaden",
address="Wiesbaden",
pages="27--33",
abstract="Ein am Institut f{\"u}r Kraftfahrzeuge der RWTH Aachen (ika) entworfenes Fahrerassistenzsystem ist in der Lage, V2X-Informationen (Vehicle-to-X) zur Optimierung der Energieeffizienz zu ber{\"u}cksichtigen. Durch die automatisierte Einleitung einer fr{\"u}hzeitigen Verz{\"o}gerung vor Signalanlagen werden unn{\"o}tige Stillstandsphasen vermieden, ohne dabei die Gesamtfahrzeit zu verl{\"a}ngern.",
isbn="978-3-658-08161-4",
}

@CONFERENCE{thomas94,
  title={Shrinking horizon model predictive control applied to autoclave curing of composite laminate materials},
  author={Thomas, Matthew M and Kardos, JL and Joseph, B},
  booktitle={Proceedings of 1994 American Control Conference-ACC'94},
  volume={1},
  pages={505--509},
  year={1994},
  organization={IEEE}
}

@ARTICLE{toh99sdpt3,
  author =       {K. C. Toh and M.J. Todd and R. H. T\"ut\"unc\"u},
  title =        {{SDPT3} - a {Matlab} software package for semidefinite programming},
  journal =      {Optimization Methods and Software},
  year =         {1999},
  volume =       {11},
  pages =        {545-581}
}

@ARTICLE{torrisi04,
  AUTHOR =       {Fabio Danilo Torrisi and Alberto Bemporad},
  TITLE =        {{HYSDEL}-A Tool for Generating Computational Hybrid Models for Analysis and Synthesis Problems},
  JOURNAL =      {IEEE Transactions on Control Systems Technology},
  YEAR =         {2004},
  volume =       {12},
  number =       {2},
}

@MISC{tosa13,
  author =       {{TOSA}},
  title =        {{Tosa flash mobility, clean city smart bus}},
  howpublished = {http://www.tosa2013.com/},
  year =         {2013},
}

@MISC{toyota,
  author =       {{Toyota Motor}},
  title =        {{Toyota Prius}},
  howpublished = {\url{http://www.toyota.com}},
  note =         {Accessed March 2012},
}

@CONFERENCE{triger93,
  AUTHOR =       {L. Triger and J. Paterson and P. Drozdz},
  TITLE =        {Hybrid vehicle engine size optimization},
  booktitle =    {SAE Future Transportation Technology Conference and Exposition, San Antonio, Texas, USA},
  YEAR =         {1993},
}

@ARTICLE{trigui04,
  AUTHOR =       {R. Trigui and B. Jeanneret and F. Badin},
  TITLE =        {System modelling of hybrid vehicles in order to predict their energy and dynamic performance: Building {VEHLIB} library},
  JOURNAL =      {Recherche Transports S�curit�},
  YEAR =         {2004},
  volume =       {83},
  pages =        {129-150},
  number =       {2},
}

@ARTICLE{tulpule10,
  AUTHOR =       {Pinak Tulpule and Vincenzo Marano and Giorgio Rizzoni},
  TITLE =        {Energy management for plug-in hybrid electric vehicles using equivalent consumption minimisation strategy},
  JOURNAL =      {Int. J. Electric and Hybrid Vehicles},
  YEAR =         {2010},
  volume =       {2},
  number =       {4},
}

@CONFERENCE{turnbull04,
  AUTHOR =       {Paul Turnbull and John Kuo and Roy Schultz and Bruce Turner},
  TITLE =        {Thermal Analysis of an Electric Machine for a Hybrid Vehicle},
  booktitle =    {SAE World Congress, Detroit, Michigan},
  YEAR =         {2004},
}

@CONFERENCE{turri14,
  AUTHOR =       {Valerio Turri and Bart Besselink and Jonas M\r{a}rtensson and Karl H. Johansson},
  TITLE =        {Fuel-efficient heavy-duty vehicle platooning by look-ahead control},
  booktitle =    {IEEE Conference on Decision and Control, Los Angeles, California, USA},
  YEAR =         {2014},
  pages =        {654-660},
}

@ARTICLE{turri16,
  title={Cooperative look-ahead control for fuel-efficient and safe heavy-duty vehicle platooning},
  author={Turri, Valerio and Besselink, Bart and Johansson, Karl H},
  journal={IEEE Transactions on Control Systems Technology},
  volume={25},
  number={1},
  pages={12--28},
  year={2016},
  publisher={IEEE}
}

% U ------------------------------------------------------------------------------------

@article{uebel17,
  title={Optimal energy management and velocity control of hybrid electric vehicles},
  author={Uebel, Stephan and Murgovski, Nikolce and Tempelhahn, Conny and B{\"a}ker, Bernard},
  journal={IEEE Transactions on Vehicular Technology},
  volume={67},
  number={1},
  pages={327--337},
  year={2017},
  publisher={IEEE}
}

@article{uebel19,
  title={A 2-Level {MPC} for Energy Management including Velocity Control of Hybrid Electric Vehicle},
  author={Uebel, Stephan and Murgovski, Nikolce and Baker, Bernard and Sjoberg, Jonas},
  journal={IEEE Transactions on Vehicular Technology},
  year={2019},
  publisher={IEEE}
}

% V ------------------------------------------------------------------------------------
@ARTICLE{vajedi15,
  title={Ecological adaptive cruise controller for plug-in hybrid electric vehicles using nonlinear model predictive control},
  author={Vajedi, Mahyar and Azad, Nasser L},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  volume={17},
  number={1},
  pages={113--122},
  year={2015},
  publisher={IEEE}
}

@ARTICLE{verscheure09,
  author =       {Diederik Verscheure and Bram Demeulenaere and Jan Swevers and Joris De Schutter and Moritz Diehl},
  title =        {Time-Optimal Path Tracking for Robots: A Convex Optimization Approach},
  journal =      {IEEE Transactions on Automatic Control},
  year =         {2009},
  volume =       {54},
  number =       {10},
  pages =        {2318-2327},
}

@inproceedings{villegas11,
  author =       {Javier Villegas and Bo Gao and Kamil Svancara and Warren Thornton and Juan Parra},
  booktitle =    {IEEE Vehicle Power and Propulsion Conference},
  pages =        {1-6},
  title =        {Real-time simulation and control of an electric supercharger for engine downsizing},
  year =         {2011},
}

@MISC{volvo,
  author =       {{Volvo Group}},
  title =        {{Volvo 7900 Hybrid Bus}},
  howpublished = {http://www.volvo.com},
  year =         {2013},
}

% W ------------------------------------------------------------------------------------
@inproceedings{wahl13,
  title={A real-time capable enhanced dynamic programming approach for predictive optimal cruise control in hybrid electric vehicles},
  author={Wahl, Hans-Georg and Bauer, Kai-Lukas and Gauterin, Frank and Holz{\"a}pfel, Marc},
  booktitle={16th International IEEE Conference on Intelligent Transportation Systems (ITSC 2013)},
  pages={1662--1667},
  year={2013},
  organization={IEEE}
}

@article{wahlstrom11,
  author =       {J Wahlstr\"om and L Eriksson},
  journal =      {Sage journals},
  number =       {7},
  pages =        {960-986},
  title =        {Modelling diesel engines with a variable-geometry turbocharger and exhaust gas recirculation by optimization of model parameters for capturing non-linear system dynamics},
  volume =       {225},
  year =         {2012},
}

@MASTERSTHESIS{wahnstrom15,
  author =       {John Wahnstr\"om},
  title =        {Energy Optimization for Platooning through Utilizing the Road Topography},
  school =       {Lund University},
  year =         {2015},
  address =      {Lund, Sweden},
}

@article{wang05,
  author =       {Jiabin Wang and Z.P. Xia and David Howe},
  journal =      {IEEE Transactions on Vehicular Technology},
  number =       {3},
  pages =        {809-816},
  title =        {Three-Phase Modular Permanent Magnet Brushless Machine for Torque Boosting on a Downsized {ICE} Vehicle},
  volume =       {54},
  year =         {2005},
}

@ARTICLE{wang11,
  AUTHOR =       {John Wang and Ping Liu and Jocelyn Hicks-Garner and Elena Sherman and Souren Soukiazian and Mark Verbrugge and Harshad Tataria and James Musser and Peter Finamore},
  TITLE =        {Cycle-life model for graphite-{LiFePO$_4$} cells},
  JOURNAL =      {Journal of Power Sources},
  YEAR =         {2011},
  volume =       {196},
  number =       {8},
  pages =        {3942-3948},
}

@ARTICLE{wei01,
  AUTHOR =       {X. Wei and G. Rizzoni},
  TITLE =        {A scalable approach for energy converter modeling and supervisory control design},
  JOURNAL =      {Proc. {ASME} Int. Mech. Eng. Congr. Expos.},
  YEAR =         {2001},
  pages =        {1281-1288},
}

@ARTICLE{wei07,
  AUTHOR =       {X. Wei and L. Guzzella and V. I. Utkin and G. Rizzoni},
  TITLE =        {Model-Based Fuel Optimal Control of Hybrid Electric Vehicle Using Variable Structure Control Systems},
  JOURNAL =      {Journal of Dynamic Systems, Measurement, and Control},
  YEAR =         {2007},
  volume =       {129},
  number =       {1},
  pages =        {13-19},
}

@TECHREPORT{wiederer10,
  AUTHOR =       {Alfred Wiederer and Ronald Philip},
  TITLE =        {Policy options for electric vehicle charging infrastructure in C40 cities},
  YEAR =         {2010},
}

@ARTICLE{williamson05,
  AUTHOR =       {Sheldon S. Williamson and Ali Emadi},
  TITLE =        {Comparative Assessment of Hybrid Electric and Fuel Cell Vehicles Based on Comprehensive Well-to-Wheels Efficiency Analysis},
  JOURNAL =      {IEEE Transactions on Vehicular Technology},
  YEAR =         {2005},
  volume =       {54},
  number =       {3},
  pages =        {856-862},
}

@ARTICLE{wipke99,
  AUTHOR =       {K.B. Wipke and M.R. Cuddy and S.D. Burch},
  TITLE =        {{ADVISOR} 2.1: A User-Friendly Advanced Powertrain Simulation Using a Combined Backward/Forward Approach},
  JOURNAL =      {IEEE Transactions on Vehicular Technology},
  YEAR =         {1999},
}

@ARTICLE{witsenhausen96,
  AUTHOR =       {H. Witsenhausen},
  TITLE =        {A class of hybrid-state continuous-time dynamic systems},
  JOURNAL =      {IEEE Transactions on Automatic Control},
  YEAR =         {1996},
  volume =       {11 (2)},
  pages =        {161-167},
}

@ARTICLE{wu11,
    AUTHOR =     {Lianghong Wu and Yaonan Wang and Xiaofang Yuan and Zhenlong Chen},
    JOURNAL =    {IEEE Transactions on Vehicular Technology},
    TITLE =      {Multiobjective Optimization of {HEV} Fuel Economy and Emissions Using the Self-Adaptive Differential Evolution Algorithm},
    YEAR =       {2011},
    volume =     {60},
    number =     {6},
    pages =      {2458-2470},
}

@article{wuX11,
    AUTHOR =     {Xiaolan Wu and Binggang Cao and Xueyan Li and Jun Xu and Xiaolong Ren},
    JOURNAL =    {Applied Energy},
    TITLE =      {Component sizing optimization of plug-in hybrid electric vehicles},
    YEAR =       {2011},
    volume =     {88},
    number =     {3},
    pages =      {799-804},
}

% X ------------------------------------------------------------------------------------

@article{xu09,
    AUTHOR =     {Liangfei Xu and Jianqiu Li and Jianfeng Hua and Xiangjun Li and Minggao Ouyang},
    JOURNAL =    {Journal of Power Sources},
    TITLE =      {Adaptive supervisory control strategy of a fuel cell/battery-powered city bus},
    YEAR =       {2009},
    volume =     {194},
    number =     {1},
    pages =      {360-368},
}

% Y ------------------------------------------------------------------------------------

@INPROCEEDINGS{yalmip,
    AUTHOR =    {J. L\"ofberg },
    TITLE =     {{YALMIP} : A Toolbox for Modeling and Optimization in {Matlab} },
    BOOKTITLE = {Proceedings of the CACSD Conference},
    YEAR =      {2004},
    URL =       {http://users.isy.liu.se/johanl/yalmip},
    ADDRESS =   {Taipei, Taiwan},
    pages =     {284-289},
}

@article{yi18,
  title={Optimal stochastic eco-routing solutions for electric vehicles},
  author={Yi, Zonggen and Bauer, Peter H},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  volume={19},
  number={12},
  pages={3807--3817},
  year={2018},
  publisher={IEEE}
}

@ARTICLE{yu16,
  author =       {Kaijiang Yu and Qing Liang and Junqi Yang and Yanan Guo},
  title =        {Model predictive control for hybrid electric vehicle platooning using route information},
  journal =      {Proceedings of the Institution of Mechanical Engineers, Part D: Journal of Automobile Engineering},
  year =         {2016},
  volume =       {230},
  number =       {9},
  pages =        {1273-1285},
}

% Z ------------------------------------------------------------------------------------

@TECHREPORT{zabat95,
  author =       {Michael Zabat and Nick Stabile and Stefano Farascaroli and Frederick Browand},
  title =        {The Aerodynamic Performance Of Platoons: A Final Report},
  institution =  {Institute of Transportation Studies, Berkeley},
  year =         {1995},
  number =       {UCB-ITS-PRR-95-35},
}

@ARTICLE{zhang10,
  AUTHOR =       {Ji-Guang Zhang and Deyu Wang and Wu Xu and Jie Xiao and R.E. Williford},
  TITLE =        {Ambient operation of {Li/Air} batteries},
  JOURNAL =      {Journal of Power Sources},
  YEAR =         {2010},
  volume =       {195},
  number =       {13},
  pages =        {4332-4337},
}

@INPROCEEDINGS{ziegler08,
  AUTHOR =       {Ziegler, J. and Werling, M. and Schr\"oder, J.},
  booktitle =    {IEEE Intelligent Vehicles Symposium},
  TITLE =        {Navigating car-like robots in unstructured environments using an obstacle sensitive cost function},
  YEAR =         {2008},
  pages =        {787-791},
}

@article{zhu18,
  title={Robust predictive battery thermal management strategy for connected and automated hybrid electric vehicles based on thermoelectric parameter uncertainty},
  author={Zhu, Chong and Lu, Fei and Zhang, Hua and Mi, Chunting Chris},
  journal={IEEE Journal of Emerging and Selected Topics in Power Electronics},
  volume={6},
  number={4},
  pages={1796--1805},
  year={2018},
  publisher={IEEE}
}

@article{zhu18real,
  title={A real-time battery thermal management strategy for connected and automated hybrid electric vehicles (CAHEVs) based on iterative dynamic programming},
  author={Zhu, Chong and Lu, Fei and Zhang, Hua and Sun, Jing and Mi, Chunting Chris},
  journal={IEEE Transactions on Vehicular Technology},
  volume={67},
  number={9},
  pages={8077--8084},
  year={2018},
  publisher={IEEE}
}

@article{zhu2018robust,
  title={Robust predictive battery thermal management strategy for connected and automated hybrid electric vehicles based on thermoelectric parameter uncertainty},
  author={Zhu, Chong and Lu, Fei and Zhang, Hua and Mi, Chunting Chris},
  journal={IEEE Journal of Emerging and Selected Topics in Power Electronics},
  volume={6},
  number={4},
  pages={1796--1805},
  year={2018},
  publisher={IEEE}
}

@ARTICLE{zoelch98,
  AUTHOR =       {U. Zoelch and D. Schroeder},
  TITLE =        {Dynamic optimization method for design and rating of the components of a hybrid vehicle},
  JOURNAL =      {International Journal of Vehicle Design},
  YEAR =         {1998},
  volume =       {19},
  number =       {1},
  pages =        {1-13},
}
